Compressed Gradient Methods with Hessian-Aided Error Compensation

The emergence of big data has caused a dramatic shift in the operating regime for optimization algorithms. The performance bottleneck, which used to be computations, is now often communications. Several gradient compression techniques have been proposed to reduce the communication load at the price of a loss in solution accuracy. Recently, it has been shown how compression errors can be compensated for in the optimization algorithm to improve the solution accuracy. Even though convergence guarantees for error-compensated algorithms have been established, there is very limited theoretical support for quantifying the observed improvements in solution accuracy. In this paper, we show that Hessian-aided error compensation, unlike other existing schemes, avoids the accumulation of compression errors on quadratic problems. We also present strong convergence guarantees of Hessian-based error compensation for stochastic gradient descent. Our numerical experiments highlight the benefits of Hessian-based error compensation, and demonstrate that similar convergence improvements are attained when only a diagonal Hessian approximation is used.

==> Introduction/compressor.tex <==
% !TeX root = ../main.tex


\section{Motivation and Preliminary Results}

In this section, we motivate our study of error-compensated gradient methods. 
First in \S~\ref{sec:Mot_Dist} we give an overview of distributed optimization algorithms  based on communicating gradient information. 
 In \S~\ref{sec:Mot_GC} we describe the general form of gradient compressions, covering most compression schemes in the literature. 
Finally in \S~\ref{sec:Mot_Low} we illustrate the limits of directly compressing the gradient, motivating the need for the error-compensated gradient method studied in this paper.
%
%
%\Sindri{When reading Section 2 and 3, I feel that the setup is not clear enough. }
%
\subsection{Distributed Optimization}~\label{sec:Mot_Dist}
%
\iffalse
\Sindri{ I feel that it would be good to set up the problem more clearly.  The problem we are studying is very simple and could be explained in a very simple way before going into details.  We are studying gradient method where gradient information is available on one node and needs to be compressed and communicated to another node.  We consider two cases: a) where full gradient information is communicated/compressed and b) where gradient is sum of partial gradients and each part is communicated/compressed separately.  
 This needs to be very clear, so we can refer to it in later sections. 
 Many people will already buy that this is a relevant setup, but for others we go into details in Sections 2.1.1 and 2.1.2.
 }\fi
%
Algorithms for distributed optimization are crucial for solving modern data-intensive applications in wireless or sensor networks, and statistical learning. This paper focuses on the minimization problem over finite average sum of several functions 
\begin{align}\label{eqn:Problem}
\mathop\text{minimize}\limits_{x\in X} \quad f(x) = \frac{1}{n}\sum_{i=1}^n f_i(x),
\end{align}
where each $f_i$ is convex and smooth, and $X\subseteq\mathbb{R}^d$ is a closed convex set.   
%
Distributed framework, where the problem \eqref{eqn:Problem} can be easily split and collaboratively executed among $m$ computing nodes, becomes the popular alternative to solve unprecedented large-scale systems over big data. One popular architecture under this framework is \emph{master-slave}, where a central node maintains the decision variable while others send the information based on local data. This architecture is proven to increase performance scalability of classical gradient-based algorithms.
%
We now review two families of gradient-based algorithms under the distributed master-slave architecture: 1) full gradient communication   and 2) partial gradient communication. 



\begin{figure}[htb]
    \centering % <-- added
\begin{subfigure}{0.5\textwidth}
\centering
  \includegraphics[width=0.3\linewidth]{D:/Papers/2018/Sindri/Figures_inkscape/full_gradientCommunication.pdf}
  \caption{}
  \label{fig:centralized}
\end{subfigure}\hfill % <-- added
\begin{subfigure}{0.5\textwidth}
  \includegraphics[width=\linewidth]{D:/Papers/2018/Sindri/Figures_inkscape/drawing.pdf}
  \caption{}
  \label{fig:distributed}
\end{subfigure}
\caption{Two scenarios of distributed learning frameworks: 1) full gradient communication (left)  and 2) partial gradient communication (right).  }
\label{fig:distributedlearningframework}
\end{figure}



%Many works propose gradient-based algorithms 

%Distributed frameworks rely on both centralized and decentralized gradient-based algorithms.

%Now, we review two common schemes for coordinating the solutions of large interconnected optimization problems based on gradient information.  


\iffalse
Recent advances in the operation of big-data and large-scale systems can be largely  traced to the successes in distributed optimization. 
 This is because sophisticated  distributed optimization algorithms have enabled multiple nodes or entities to collaboratively  solve large interconnected problems with the problem data split between them. 
  To implement these algorithms,  nodes need to communicate some information, typically gradients or subgradients, among themselves.  
  We now review two common schemes for coordinating the solutions of large interconnected optimization problems based on gradient information.   
\fi
%
% 
%  A key ingredient in these algorithms is the communication between the nodes and 
%  Distributed optimization algorithms have allowed multiple parties to solve huge problems that are separated between them.  
%  Often the information that is communication are gradients of some of the related functions, of either the primal or dual dual function

\subsubsection{Full Gradient Communication: Dual Decomposition} \label{sec:Mot_Dist1}

\emph{Resource allocation} is the modern distributed optimization problem, where a group of $n$ agents aims to minimize the utility function over coupled/shared constraints (\emph{e.g.}, resource limitations). In particular, all agents collaboratively solve 
\begin{equation} \label{EQ:ProblemFullGradient}
\begin{aligned}
& \underset{q_1,\ldots,q_n}{\text{minimize}}
& & \sum_{i=1}^n U_i(q_i)\\
& \text{subject to}
& & g(q_1,q_2,\ldots,q_n)\leq 0, \\  %~~(\text{or } g(q_1,\ldots,q_N )\leq 0)\\
&&& q_i\in \mathcal{Q}_i,~~i=1,\ldots,n.
\end{aligned}
\end{equation}
Here, each agent has the private utility function $U_i(q_i)$, the private decision variable $q_i$ and the private constraint set $\mathcal{Q}_i$. The decision variables are coupled with the constraint $g(q_1,q_2,\ldots,q_n)\leq 0$, which captures physical or economical limitations. 

The resource allocation problems often arise in wireless networks, data communications, power systems and smart grids. For instance, we are interested in optimizing the data flow between $n$ destination pairs through an $L-$link communications network by  solving the following utility minimization problem
%
 \begin{equation} \label{EQ:TCP}
\begin{aligned}
& \underset{q_1,\ldots,q_n\in \mathbb{R}}{\text{minimize}}
& & \sum_{i=1}^n U_i(q_i)\\
& \text{subject to}
& & \sum_{i\in S_l}^n q_i \leq c_l, ~~~l=1,\ldots,L\\  %~~(\text{or } g(q_1,\ldots,q_N )\leq 0)\\
&&& q_i\in [\underline{q}_i,\bar{q}_i]~~i=1,\ldots,n.
\end{aligned}
\end{equation}
 where  $\mathcal{S}_l$ is a set containing the source/destination pairs that use link $l$. 
 Here the local functions $U_i(\cdot)$ models the  the economic utility of the data to each user or fairness or priority between the different source/destination pairs when allocating the data. 
%  Similarly, in wireless networks, we can optimize data-rates while using shared  there the coupling constraints  optimize  utilities and constraints further model collations package-drop 
 In electric power systems, we focus on optimizing power usage or consumption over a group of electric devices (\emph{e.g.}, smart meters, household appliances and renewable generators) by solving the power utility minimization problem \eqref{EQ:ProblemFullGradient} with $g(q_1,q_2,\ldots,q_n)=\sum_{i=1}^n q_i$ and $\mathcal{Q}_i = [\underline{q}_i,\bar{q}_i]$.
 
 
Dual decomposition methods are commonly used to solve the resource allocation problem \eqref{EQ:ProblemFullGradient},~\cite{}. These methods rely on leveraging the problem among the coordination of agents which solve subproblems and communicate the gradient information,~\cite{}. To illustrate the procedure, we rather consider the following dual problem equivalent to \eqref{EQ:ProblemFullGradient}
\begin{equation} \label{EQ:ProblemFullDual}
\begin{aligned}
 & \underset{\lambda\geq 0}{\text{maximize}}
& & D(\lambda):= \min_{q} L(q,\lambda). %\\
%&&& \lambda \geq 0
\end{aligned}
\end{equation}
 where  $\lambda$ is the dual variable, $D(\lambda)$ is the dual objective function,  and  %is the given by
% To construct the dual problem we consider the Lagrangian function
$$L(q,\lambda)= \sum_{i=1}^n U_i(q_i)+\lambda^T g(q_1,\ldots,q_n ),$$
is the Lagrangian of the Problem~\eqref{EQ:ProblemFullGradient}.
%where  $\lambda$ is the dual variable.  The dual function  % is
%$$ D(\lambda)= \min_{q} L(q,\lambda)$$
 The dual function is concave and the dual gradient (or a dual subgradient) is given by
 $$\nabla D(\lambda)= g(q_1(\lambda),\ldots,q_n(\lambda) ),~~~~q(\lambda)=\underset{q}{\text{argmin}}\, L(q,\lambda).$$
 Therefore, we solve the equivalent dual problem \eqref{EQ:ProblemFullDual} by the projected gradient method
 \begin{align*}
         q_i^{k+1}=&\underset{q}{\text{argmin}} ~U_i(q_i^k) +(\lambda^k)^T  g_i(q_i^k) , ~~~~i=1,\ldots,n \\
       \lambda^{k+1} =&  \left\lceil \lambda^k+\gamma
         g(q_1^{k+1},\ldots,q_n^{k+1} )\right\rceil_+
 \end{align*}
 where $\gamma$ is the fixed, positive step-size.  
% If performing the optimization in computing $q^{k+1}$ is difficult then we might consider taking a gradient step also for the primal variable:
% \begin{align*}
%         q_i^{k+1}=& q^{k} - \gamma\left( \nabla U_i(q_i) +\sum_{i=1}^n \lambda_i^k  \nabla g_i(q_i^k) \right) , ~~i=1,\ldots,n
%       \\%=& \left\lceil \lambda^k+\gamma \nabla D(\lambda^k) \right\rceil_+ 
%       \lambda^{k+1} =&  \left\lceil \lambda^k+\gamma 
%         g(q_1^{k+1},\ldots,q_n^{k+1} )\right\rceil_+ .
% \end{align*}
Notice that the essential step for coordination among agents is to communicate the dual gradients $g(q_1^{k+1},\ldots,q_n^{k+1})$ so that each agent can update $q_i^{k+1}$ based only on the global dual variable $\lambda^k$.



 %
 \iffalse
 many variants of the  optimization problem in Equation~\eqref{EQ:ProblemFullGradient} are used to ensure efficient and economical operation. 
 Traditionally, such optimization has mainly been performed in high-voltage transmission networks that transport electricity long distances between few large stakeholders, e.g., large power plants and large industrial consumer. 
 However, with increased automation, distributed optimization is starting to have large impact in low voltage distribution networks were devices such as smart meters, smart home appliances, and renewable generators  collaboratively optimize the grids performance. 
   % Optimization problems in power systems range with the simplest one being Economic Dispatch: 
   The simplest optimization problem  typically considered in power systems is economic dispatch, 
%   \begin{equation} \label{EQ:TCP}
%\begin{aligned}
%& \underset{x}{\text{minimize}}
%& & \sum_{i=1}^n U_i(q_i)\\
%& \text{subject to}
%& & \sum_{i=1}^n q_i =0, \\  %~~(\text{or } g(q_1,\ldots,q_N )\leq 0)\\
%&&& q_i\in \mathcal{Q}_i,~~i=1,\ldots,n.
%\end{aligned}
%\end{equation} 
 where $q_i\in  [\underline{q}_i,\bar{q}_i]\subseteq \mathbb{R}$
 is the power usage or consumption of node/device $i$  and the coupling constraint  
 $$ \sum_{i=1}^n q_i =0$$
 ensures power balance, i.e., that supply equals demand.  
 The economic dispatch problem is a crude simplification of physics of the power system. 
 More detailed modeling can be included in the constraint  $g(q_1,\ldots,q_n)\leq 0$ such as power flows were local variables $q_i$ are vectored value keeping the  real/reactive powers, currents, and voltages.
\fi

\iffalse
\SK{In dual decomposition, the dual to an optimization problem with a specific structure is solved in distributed fashion using classical gradient descent. }


\SK{Details on dual decomposition and how to apply full gradient descent} 

 
 
Many distributed optimization problem include multiple nodes that have coupled constraints or shared resources. Representative examples can be found in wireless networking, data communication, power systems, and sensor networks, to mention a few. 
  These problems are typically solved by dual decomposition methods where the nodes communicate dual gradients to coordinate the system-wide problem. 
 % Distributed optimization algorithms that have coupled constraints are typically addressed by dual decompensation methods were based on communicating dual gradients.
% 
% These methods solve
 To illustrate this process consider the following optimization problem: %, if we consider optimization on the following 


Here there are $n$ nodes, $i=1,\ldots,n$, each with a local objective/utility function  $U_i(q_i)$ and a private decision variable $q_i$, and private constraint set $\mathcal{Q}_i$. 
The decision variables are coupled by the constraint  $g(q_1,\ldots,q_n)\leq0$, capturing the physical/economical limitations or shared some resources.
 In communication networks, optimization problems of the form of Equation~\eqref{EQ:ProblemFullGradient} are used to optimize  data-flows in wired networks and allocate radio resources such as bandwidths, time slots, and data rates in wireless networks. 
 For example, in wired network we are often interested in optimizing the flow of data between $n$ source/destination pairs through a $L$-link network  by solving the following optimization problem:


 
We are interested in distributed algorithms for solving problems of the form of Equation~\eqref{EQ:ProblemFullGradient}. 
The coupling constraint  $g(q_1,\ldots,q_n)\leq0$ inhibits the nodes to find the network-wide optimal solution by simply minimizing their their local objective function.  
This means that the nodes need to coordinate to solve the optimization problem.
 This coordination  is typically based on communicating the gradient  of the dual problem. 
 To illustrate this process, we consider the dual problem
\fi
%
%
\subsubsection{Partial Gradient Communication}

Another setting that often arises in distributed optimization is where $m$ nodes/agents wish to solve Problem \eqref{eqn:Problem}. 
%
%the sum of local objective functions as follows:
%In this paper,  we consider the minimization problem over the average of a large number of smooth, differentiable functions
%\begin{align}\label{eqn:Problem}
  %  \mathop{ \text{minimize}}\limits_{x\in\mathbb{R}^d} \quad f(x) = \frac{1}{m}\sum_{i=1}^m f_i(x).
%\end{align}
%
%
%Problem \eqref{eqn:Problem}, also known as \emph{empirical risk minimization} (ERM), arises in machine learning, statistics and signal processing. This problem includes least-squares estimation, logistic regression, and support vector machines.
%Here the objective function $f_i(x)$ is maintained locally by node $i$
 An instance of  this problem that frequently arises in machine learning, statistics and signal processing is distributed \emph{empirical risk minimization} (ERM). There, these $m$ nodes wish to collaboratively  find global optimal estimators based on labelled  data that is separated among them.
 For example,  if each node $i=1,\ldots,n$ has accesses its local data with feature vectors $\vec{z}_i=(z_i^1,\ldots,z_i^m)$ and labels $\vec{y}_i=(y_i^1,\ldots,y_i^m)$ with $z_i^j\in \mathbb{R}^d$ and $ y_i^j\in \mathbb{R}$, then local objective functions of the $\ell_2$-regularized ERM~\eqref{eqn:Problem} has the form
%
%
\begin{align}\label{eqn:fi_ERM}
f_i(x)=\frac{1}{m}\sum_{j=1}^m \ell(x; z_i^j,y_i^j)+ \frac{\lambda}{2}||x||_2^2, \quad \text{for } i=1,2,\ldots,n
\end{align}
%
%
where $\ell(\cdot)$ are some loss functions and $\lambda>0$ is the $\ell_2-$regularizer. Depending on estimation applications, examples of the loss function include:
\begin{itemize}
\item Ridge regression: $\ell(x; z,y)= \frac{1}{2} (y- z^T x)^2.$
\item Hinge loss: $\ell(x; z,y)= \max\{0,1-y\cdot z^T x \}.$
\item Logistic regression: $\ell(x; z,y)=\log(1+\exp(-y\cdot z^T x)).$
\end{itemize}
 
\iffalse 
For example, in ridge regression, 
\ell(x; z,y)= \frac{1}{2} (z^T x-y)^2,$$
support vector machines use
$$\ell(x; z,y)= \max\{0,1-y\cdot z^T x \},$$
and logistic regression is defined by 
$$\ell(x; z,y)=\log(1+\exp(-y\cdot z^T x).$$
\fi 



For unprecedented huge-scale data sets, modern engineering applications focus on solving Problem \eqref{eqn:Problem} when $m$ is extremely large. \emph{Stochastic gradient descent} (SGD) is among the most popular randomized first-order algorithms, since it enjoys a low per-iteration cost and small memory footprints, \cite{needell2014stochastic}. Even though theoretically and empirically proven to have near-optimal computational complexity by proper step-size tuning \cite{needell2014stochastic}, SGD has severely limited performance scalability by its  inherently sequential computation. 

One simple modification is \emph{mini-batching}, which processes several samples per iteration and allows to reduce the variance of gradient estimates. Mini-batch SGD takes smaller iteration counts and enjoys significantly low training time, since it can easily utilize massive parallelization to attain high scalability by modern multi-core processors, or even by computer clusters. In each iteration of mini-batch SGD under distributed frameworks, the master node typically broadcasts a decision variable $x^k$, while each worker node $i$ queries a stochastic gradient 
$\nabla g_i(x^k;\xi_i^k)$ with the random index $\xi_i^k$ selecting part of its local data $\mathcal{D}_i$. After the master  receives the information from all worker nodes, it can perform the update
%
%
% 
\begin{align}\label{eqn:minibatchSGD}
x^{k+1}=x^k-\gamma \frac{1}{n}\sum_{i=1}^n \nabla g_i(x^k;\xi_i^k).
\end{align}
Here, the stochastic gradient preserves unbiased property, i.e. 
\begin{align}
\mathbb{E}_{\xi_i} \nabla g_i(x;\xi_i) = \nabla f_i(x), \quad \forall x\in\mathbb{R}^d.
\end{align}
For the $\ell_2-$regularized ERM, $\nabla g_i(x;\xi_i) = (1/|\mathcal{B}_i|)\sum_{j\in \mathcal{B}_i}\nabla \ell(x;z_i^j,y_i^j) + \lambda x,$ where the mini-batch $\mathcal{B}_i$ is the subset of data $\mathcal{D}_i$ of size $|\mathcal{B}_i|$ at worker node $i$, which is selected uniformly at random. 

Even though many works proved the convergence rate of distributed mini-batch SGD \cite{lian2017can,lian2015asynchronous,feyzmahdavian2016asynchronous,alistarh2017qsgd}, they assume similarity between local data distributions $\mathcal{D}_i$ and the whole data distribution $\cup_{i=1}^m \mathcal{D}_i$. The results imply significantly slow convergence of distributed mini-batch SGD even with low solution accuracy since the cluster in practice contains computer nodes with too different computing performance and memory requirements.  Following \cite{mishchenko2019distributed}, our analysis admits highly heterogeneous data distributions among the worker nodes. To further limit the amount of data exchanged in these distributed algorithms, it has been suggested to compress or quantize the gradients before they are communicated. 
%accomplish these distributed algorithms some communication is needed, which generally requires some %compression or distortion of the communication gradients. 
We now review the compression schemes we consider in this paper. 



 



\iffalse
For large-scale datasets, Problem~\eqref{eqn:Problem} is solved in a distributed manner where a master node coordinates the executation of a first-order method, typically gradient descent or stochastic gradient descent. 
To that end, the master node typically broadcasts a decision variable $x^k$ at each iteration, while
each node  $i$ communicates back either the gradient $\nabla f_i(x^k)$ based on the full local data at node $i$ or a stochastic gradient based on part of the data (a mini-batch) at node $i$. 
\fi

\iffalse
To limit the amount of data exchanged in these distributed algorithms, it has been suggested to compress or quantize the gradients before they are communicated. 
%accomplish these distributed algorithms some communication is needed, which generally requires some %compression or distortion of the communication gradients. 
We now review the compression schemes we consider in this paper. 
\fi

\subsection{Gradient Compression} \label{sec:Mot_GC}
%This section introduces two families of generic compression operators.


Under distributed learning frameworks, communication costs of the exchange of gradient vectors among computer nodes within a cluster can easily lead to significant performance limitations especially for problems with huge dimension.  One common way is to compress the gradient vector before broadcasting it into a finite precision which can be represented by a few numbers of communicated bits. 
%
%
%
\iffalse
In practice we need to compress the gradient vectors to finite precision before we can communicate them. % communication  it generally needs to be compressed.  
 For example, to implement the  full gradient methods in Subsection~\ref{sec:Mot_Dist1}  we need to compress the gradient $\nabla f(x)$, resulting in the compressed gradient method % version of the gradient $\nabla f(x)$, instead of the gradient itself. 
 \begin{equation} \label{eq:CompressedGradient} 
    x^{k+1}=x^k-\gamma Q(\nabla f(x^k))
 \end{equation}
  where $Q(\nabla f(x^k))$ is a compression operator that maps the gradient to finite precision.  More agressive  compression  leads to smaller data exchange but also lower precision.
 \fi 
%  
% 
% do note communicate the gradient $\nabla f(x)$ itself, but instead we co is communicated we compressed it with some
%
In this paper, we study a wide range of compression schemes and an  error-compensation mechanism that work well on all of them.  In particular, we consider both deterministic and stochastic compression operations defined as follows.
%
%
%
%
\begin{definition}\label{def:DBEC}
The operator $Q:\mathbb{R}^d\rightarrow\mathbb{R}^d$ is an $\epsilon-$\emph{deterministic compressor} if there exists a positive constant $\epsilon$ such that
\begin{align*}
\| Q(v) - v \|^2 \leq \epsilon, \quad \forall v\in\mathbb{R}^d.
\end{align*}
\end{definition}



Unlike \cite[Definition 2.1]{Stich2018} and \cite[Assumption A]{2019arXiv190109847P}, Definition \ref{def:DBEC} allows for compressors to have  quantization error arbitrarily larger than magnitude of the original vector.


\begin{definition}\label{def:UBEC}
The operator $Q:\mathbb{R}^d\rightarrow\mathbb{R}^d$ is an $\epsilon-$\emph{stochastic compressor} if for all $v\in\mathbb{R}^d$
\begin{enumerate}
\item $\mathbf{E} \{Q(v)\} = v$, and 
\item $\mathbf{E}\| Q(v) - v \|^2 \leq \epsilon$ 
\end{enumerate}
for some positive constant $\epsilon$. 
\end{definition}


According to Definition \ref{def:DBEC} and \ref{def:UBEC}, a low value of $\epsilon$ implies high compression accuracy ($\epsilon=0$ when $Q(v)=v$).
The definitions above cover many compressors of practical interest, which substantiates the generality of our results later in the paper. For example, the rounding quantizers are as defined below:  


%{\color{red} \textbf{Sindri:} I prefer not to have the examples of compressions as definitions, it makes the message
\begin{example}[\cite{li2017training,rabbat2005quantized,zhu2016quantized}]\label{def:deterRQ}
For a given quantization resolution $\Delta >0$, the \emph{deterministic rounding quantizer} $Q_{dr}:\mathbb{R}^d\rightarrow\Lambda$ is defined as
\begin{align*}
[Q_{dr}(v)]_i &= {\rm sign}(v_i) \cdot \Delta\cdot \floor*{ \frac{|v_i|}{\Delta} +\frac{1}{2}}, 
\end{align*}
where $v\in\mathbb{R}^d$.
\end{example}



\begin{example}[\cite{li2017training}]
\label{def:stochRQ}
For a given quantization resolution $\Delta>0$, the  \emph{randomized rounding quantizer} $Q_{sr}:\mathbb{R}^d\rightarrow\Lambda$ is defined as
\begin{align*}
[Q_{sr}(v)]_i & = \left\{\begin{array}{ll} \Delta\left(\floor*{\frac{v_i}{\Delta}} + 1\right) &  \text{with probability} \quad p = \frac{v_i}{\Delta} - \floor*{\frac{v_i}{\Delta}} \vspace{0.2cm}\\
 \Delta\floor*{\frac{v_i}{\Delta}} & \text{otherwise}    \end{array}\right. , 
\end{align*}
where $v\in\mathbb{R}^d$.
\end{example}

It is easy to show that the deterministic and randomized rounding quantizer are 
$\epsilon-$deterministic and $\epsilon-$stochastic compressors with $\epsilon = d\cdot\Delta^2/4$ and $d\cdot \Delta^2$, respectively, \cite{rabbat2005quantized,zhu2016quantized,li2017training,de2018high}. 
%
%
In addition, it is worth mentioning that Definitions \ref{def:DBEC} and \ref{def:UBEC} cover popular compressors or quantizers in machine learning and control theory appplications. If we assume bounded gradient assumptions and apply the compressor to gradients, then it is easy to prove that the $\epsilon$-deterministic compressor covers the $K-$greedy quantizer \cite{gradientcompression2018} and the dynamic gradient quantizer \cite{gradientcompression2018,alistarh2017qsgd}, while the $\epsilon-$stochastic compressor covers the gradient sparsifier \cite{wangni2017gradient} and the low-precision quantizer \cite{khirirat2018distributed,alistarh2017qsgd}. 



% some sentences saying that making the bounded gradient assumptions implies definitions of our compressors include these results. 

%\begin{itemize}
%	\item Perhaps mention something about other quantizers under bounded gradient assumption?
%\end{itemize}

\subsection{Direct Gradient Compression: Lower Bounds and Convergence}\label{sec:Mot_Low}

%\begin{itemize}
%	\item Add some introductory glue text here\dots 
%\end{itemize}

\Sindri{From my comment below, I think it is good to move all discussion and theorems on directly compressing the gradient here. That way we can keep the next section very clean and go directly to the main message and results. I have tried to move the writing of this section towards this direction, but we need to work on a bit more.}

Even though SGD with many compressors is shown to enjoy savings in per-iteration communication costs, and to converge with the same theoretical and empirical rate as full-precision SGD in deep learning applications, too crude compressions which are naively applied on optimization algorithms can often slow down convergence with significant solution inaccuracy. To show that this intuition is correct, this section studies compressed gradient descent (CGD) which forms the following iteration: given the positive step-size $\gamma$, and the initial point $x_0\in\mathbb{R}^d$
%
%
\begin{align}\label{eqn:CGD}
x_{k+1} = x_k - \gamma Q\left( \nabla f(x_k) + \omega_k \right),
\end{align}
where $\omega_k$ is the stochastic noise satisfying $\mathbf{E}\omega_k=0$ and $\mathbf{E}\| \omega_k\|^2 \leq \sigma^2$. CGD \eqref{eqn:CGD} often appears as common techniques applied on dual decomposition methods to solve resource allocation problems in wireless network applications (see details in Section \ref{sec:Mot_Dist1}).


To this end, we show a simple example when applying the $\epsilon-$deterministic compressor, and argue that error compensation scheme is a necessary solution.  



\iffalse
When provided quantization function $Q(\cdot)$ for compressing the communicated gradient information, 
 it is  most straightforward to directly compress the  gradient. 
%To this end, we start by studying compressed gradient descent (CGD) which forms the following iteration
%
%
 The result gradient method would be
\begin{align}\label{eqn:CGD}
x_{k+1} = x_k - \gamma Q\left( \nabla f(x_k) \right).
\end{align}
 Since we use the compressed gradient step $Q(\nabla f(x_k) )$   suggests  that we should suffer some inaccuracies in our solution.  
%  When we perform gradient methods with compressed gradients, as we did in Equation~\eqref{eq:CompressedGradient}, then intuition  suggests  that we should suffer some inaccuracies in our solution.  
  For example, if our quantizer is $\epsilon$-DBEC then we might suspect that our algorithm could only provide us with a sub-optimal solution and that the quality of the solution should be somehow related to $\epsilon$. 
  We now show that this intuition is correct  with a simple example. Will illustrate how to fix this behavior with a simple gradient correction in the next section. 
 \fi
% this h. % We illustrate of to correct for this behavior in providing our correcting scheme that fixes this behavior. 
%  
%   the gradient it is expected that we loose some information, and  such as the gradient is expected
%  
%This section studies the limitations of naive gradient compression. Under commonly-used assumptions of loss functions, gradient-based optimization algorithms converge toward the sub-optimum due to quantization noises; see \emph{e.g.}, in \cite{khirirat2018distributed}. By the simple quadratic optimization problem, we further demonstrate that simple gradient compression cannot make solution accuracy lower than a certain threshold. 


\begin{example}\label{ex:SimpleQ}
\textit{
Consider the scalar optimization problem
\begin{equation*}
\begin{aligned}
& \underset{x}{\text{minimize}}
& &  \frac{1}{2} x^2.
\end{aligned}
\end{equation*}
 Suppose that we run the compressed gradient decent algorithm with $\omega_k=0$:
 \begin{align} \label{eq:quant_gradient}
   x^{k+1}=x^k-\gamma Q(f'(x^k))=x^k-Q(x^k),
 \end{align}
 where $Q(\cdot)$ is the $\epsilon$-DBEC compression (see Definition~\ref{def:DBEC})\footnote{\textbf{Sindri:} I define $Q(\cdot)$ using $z/|z|$ rather than the $\texttt{sign}(\cdot)$ function because the generalization to higher dimension is $z-\epsilon z/||z||$ rather than $z-\epsilon \texttt{sign}(z)$.}
 $$Q(z)= \begin{cases} z-\epsilon \frac{z}{|z|} &\text{if } z\neq 0 \\ \epsilon & \text{otherwise}. \end{cases}  $$ %\texttt{sign}(z),$$
 %where $\texttt{sign}(z)=z/|z|$ if $z\neq 0$ and $\texttt{sign}(0)=1$. 
% $$|Q(z)-z|\leq \epsilon~~\text{ for all }~~ z\in \R.$$
% This condition holds for $Q(z)=z-\epsilon$ and with this $Q(\cdot)$, 
If we  take $\gamma\in (0,1]$  and $|x^0|>\epsilon$ then for all $k\in \mathbb{N}$ we have
 \begin{align*}
    |x^{k+1}-x^{\star}|=|x^{k+1}|=&|x^k-\gamma Q(f'(x^k))|\\
     %=&x^k-\gamma(x^k-\epsilon) \\
     %=&  |(1-\gamma) x^k+\gamma\epsilon |\\
     =&  (1-\gamma) |x^{k}|+\gamma\epsilon \\
     =&  (1-\gamma)^{k+1} |x^0| + \epsilon \gamma \sum_{i=0}^k (1-\gamma)^i \\
     =&  (1-\gamma)^{k+1} |x^0| + \epsilon \gamma \frac{1-(1-\gamma)^{k+1}}{\gamma} \\     
     =&  (1-\gamma)^{k+1}(|x^0|-\epsilon)+ \epsilon \\
     \geq& \epsilon,
 \end{align*}
% \begin{align*}
%    |x^{k+1}-x^{\star}|=x^{k+1}=&x^k-\gamma Q(f'(x^k))\\
%     =&x^k-\gamma(x^k-\epsilon) \\
%     =&  (1-\gamma) x^k+\gamma\epsilon \\
%     =&  (1-\gamma) x^{k}+\gamma\epsilon \\
%     =&  (1-\gamma)^{k+1} x^0 + \epsilon \gamma \sum_{i=0}^k (1-\gamma)^i \\
%     =&  (1-\gamma)^{k+1} x^0 + \epsilon \gamma \frac{1-(1-\gamma)^{k+1}}{\gamma} \\     
%     =&  (1-\gamma)^{k+1}(x^0-\epsilon)+ \epsilon \\
%     \geq& \epsilon,
% \end{align*}
 where we have used that $x^{\star}=0$.\footnote{\textbf{Sindri:} It would be nice to also have some lower bound for the UBEC compression.}
 }

 \end{example}
 By the above example, we can show that the $\epsilon$-deterministic compressor cannot achieve better than $\epsilon$ accuracy.  However, in this paper we show the surprising fact that an arbitrarily  good accuracy can indeed be obtained even when the the gradient information compressed by the $\epsilon$-deterministic compressor if we include a simple correction step in our compressed gradient method.
 
\Sindri{I suggest putting Theorem 1 and 2 here.  It is good if the upper bounds match the lower bound  well.  For example, now Theorem 1 and 2 use stochastic compression but the lower bound uses deterministic compressor. I think if we use the deterministic compressor then we can match the upper and lower bound.  We could give the example and then have one theorem with 3 cases: a) Strongly convex, b) convex and smooth (convergence in objective function value), c) smooth (convergence of gradient). In each case we could say, and there exists a function $f(\cdot)$ such that the bound holds with equality, then in the proof we use the example above and explain that also after giving the theorem. }
 
 
\SK{So far, it is simply possible to show the convergence rate of compressed SGD with diminishing step-sizes for strongly convex and non-convex optimization.}
 
 
Finally, we provide the convergence rate results of CGD with the $\epsilon$-stochastic compressor. 
 
\begin{theorem}\label{thm:CGDimproved}
Consider an optimization problem \eqref{eqn:Problem} and the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:CGD}. Assume that the compressor is the $\epsilon-$stochastic compressor and that $\gamma < 1/L$. If the whole objective function $f$ is $L-$smooth, then  
\begin{align*}
\mathbf{E} \| \nabla f(x_l) \|^2 \leq \frac{1}{k+1} ...
\end{align*}
In addition, if $f$ is convex, then
\begin{align*}
\mathbf{E} f(\bar x_k) - f(x^\star) \leq \frac{1}{k+1} ...
\end{align*}
\end{theorem}
\begin{proof}
See Appendix ... 
\end{proof}


Theorem \ref{thm:CGDimproved} establishes the sub-linear convergence rate of CGD with the $\epsilon-$stochastic compressor, unlike $\epsilon-$deterministic compressor. Also, we recover the convergence of classical gradient descent when we let $\epsilon=0$ in Theorem \ref{thm:CGDimproved}. However, we show that the error compensation scheme indeed helps improve solution accuracy in the next section.



 

 \iffalse
  The above example shows that even for the most simple of optimization problems, strongly convex quadratic scalar problem, the $\epsilon$-DBEC compression can not achieve better than $\epsilon$ accuracy.  
  This fact is probably not surprising, we had already predicted it. 
  However, in this paper we show the surprising fact that an arbitrarily  good accuracy can indeed be obtained even when the the gradient information compressed by $\epsilon$-DBEC if we include a simple correction step in our compressed gradient method.
 \fi
  

  
  %\footnote{\textbf{Sindri:} I like this ending because it is kind of a cliffhanger, makes the reader curios to continue to the next section.   So I was thinking if it is good to call the next section something like: \emph{Main Results: Error Compensated Gradient Compression} and start by giving the over all scheme and then split into the two subsection Full gradient Compensation and Partial Gradient Compensation. }  
  
 
  









==> Introduction/compressor_SK_1.tex <==
% !TeX root = ../main.tex
%
%
\section{Motivation and Preliminary Results}
%
%
In this section, we motivate our study of error-compensated gradient methods. 
First in \S~\ref{sec:Mot_Dist} we give an overview of distributed optimization algorithms  based on communicating gradient information. 
 In \S~\ref{sec:Mot_GC} we describe the general form of gradient compressions, covering most compression schemes in the literature. 
Finally in \S~\ref{sec:Mot_Low} we illustrate the limits of directly compressing the gradient, motivating the need for the error-compensated gradient method studied in this paper.
%
%
\subsection{Distributed Optimization}~\label{sec:Mot_Dist}
%
Distributed optimization algorithms have enabled  us to solve large-scale and data-intensive problems in a wide range of application areas such as smart grids, wireless networks, and statistical learning. Many distributed optimization algorithms build on gradient methods and can be categorized based on whether they use a) full gradient communication and b) partial gradient communication, as shown in Figure \ref{fig:distributedlearningframework}. The full gradient communication algorithms solve problems on the form
 \begin{align}\label{eqn:Problem}
\mathop\text{minimize}\limits_{x} \quad f(x), %= \sum_{i=1}^n f_i(x),
\end{align}
 by performing a standard gradient method %\Sindri{To be consistent, we can remove the constraints and projection here.}
 \begin{align}\label{eqn:FullGDcentralized}x^{k+1}= x^k-\gamma \nabla f(x^k),\end{align}
  where the full gradient $ \nabla f(x^k)$ is communicated at every iteration.
   Such communication usually appears in dual decomposition methods where $f(\cdot)$ is a dual function associated with some large-scale primal problem, we illustrate this in subsection~\ref{sec:Mot_Dist1}. 
 The partial gradient communication algorithms solve separable optimization problems among $n$ nodes  on the form
 \begin{align}\label{eqn:Problem}
\mathop\text{minimize}\limits_{x} \quad f(x) = \frac{1}{n}\sum_{i=1}^n f_i(x),
\end{align}
 %
%
 %
 %
  by  performing a separable gradient method
  \begin{align}x^{k+1}=x^k-\frac{\gamma}{n} \sum_{i=1}^n \nabla f_i(x^k) , \label{eqn:fulldistGD}\end{align}
   where each partial gradient $\nabla f_i(x^k)$ is communicated by node $i$ (see subsection~\ref{subsec:PartialGradient}). % needs to communicates its gradient $\nabla f_i(x^k)$. 
  Clearly, the full gradient communication is a special case of the partial gradient communication with $n=1$.  
  However, considering the full gradient communication algorithms separately  will enable us to get stronger results in that case. We now review these algorithms separately in the next subsections.
  %
%  a) Full gradient communication architecture where the full gradient $\nabla f(x)$ is communicated at every iteration and b) partial  gradient communication architecture where 
% $$f(x)=\sum_{i=1}^n f_i(x),$$
% .  We review these two communication architectures, respectively, in the next two subsections. 






















%%%%%%%%%%%%%%%%%%%%%%%%%% OLD TEXTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% OLD TEXTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% OLD TEXTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% OLD TEXTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Distributed optimization algorithms have enabled  us to solve large-scale and data-intensive problems in wide range of application areas such as smart grids, wireless networks, and statistical learning. These algorithms are typically used to solve  minimization problems   
 over finite average sum of several functions on the form
\begin{align}\label{eqn:Problem}
\mathop\text{minimize}\limits_{x\in X} \quad f(x) = \frac{1}{n}\sum_{i=1}^n f_i(x),
\end{align}
where each component function  $f_i$ can be eiter convex or nonconvex, and and $X\subseteq\mathbb{R}^d$ is a closed convex set.   
%
{\color{red}
Distributed framework, where the problem \eqref{eqn:Problem} can be easily split and collaboratively executed among $m$ computing nodes, becomes the popular alternative to solve unprecedented large-scale systems over big data. One popular architecture under this framework is \emph{master-slave}, where a central node maintains the decision variable while others send the information based on local data. This architecture is proven to increase performance scalability of classical gradient-based algorithms.
We now review two families of gradient-based algorithms under the distributed master-slave architecture: 1) full gradient communication   and 2) partial gradient communication. }

\Sindri{ Regarding the above paragraph:
\begin{itemize}
  \item  
  We have already a natural splitting of the problem into $n$ objective functions. Now you want to split that problem up between $m$ computing nodes, it is a bit confusing.  For now we don't need to go into details on how the data is splits between the computing nodes for particular problems. It is better to make this discussion general and discuss specific implementations later.  %We can just say: we have $n$ nodes each with a local objective function and we like to minimize the sum  of the local objective functions. This is the general setting we consider. % "where
  % We then discuss the statistical learning and how we split different data points between different computing nodes in subsection 3.1.1. 
  \item What is a distribution framework? it is a bit obscure.  
  %
  \item The paragraph is not conveying the main message: 1) Gradient methods where a gradient is communicated at every iterations is the building block of many distributed algorithms 2) there are two common communication arcitecture for performing these distributed gradient methods a) communicating full gradient and b) communicating partial gradients. We review these two architectures in the sequel. 
  \item The paragraph is to focussed on the learning application, Section 3.1.1 discusses smart grids and communication networks, there are no $m$ data points there. For these applications it is a bit strange to talk about master-slave architecture. Also even for the master-server case we don't always have data points.  Lets try to make this discussion general and then give application example in the subsection.
  \item Notice how the flow is not good, there is no talk of any gradient methods until suddenly in the end when it is reveal that the whole paragraph was about gradient methods.
  \item I changed the optimziation problem. Earlier it only included the optimization problem for the partial gradient method.
  % It needs to be general so it covers both the full gradient communication and partial communication arcitectures. 
\end{itemize}
Here is my revised paragraph:
}


\SM{Distributed optimziation algorithms have enabled  us to solve large-scale and data-intensive problems in wide range of application areas such as smart grids, wireless networks, and statistical learning. %These algorithms are used to solve optimiation problems, such as %, such as % like that are naturally decomposed between $n$ nodes,  frequently   on the form
%\begin{align}\label{eqn:Problem}
%\mathop\text{minimize}\limits_{x\in X} \quad f(x), %= \sum_{i=1}^n f_i(x),
%\end{align}
%that can somehow be naturally decomposed between multiple nodes.  
%where the function $f_i$ is kept by node $i$.  
% A building block for many distributed optimization algorithms are based on 
 Many distributed algorithms build on gradient  methods where some gradient information is communicated  over the course of the algorithm. % are usually  methods 
 These distributed gradient methods can generally be split into two categories based on the gradient information they communicate: a) full gradient communication and b) partial gradient communication. 
%  Algorithms that use full gradient communication are simply gradient methods
%   $$x^{k+1}=\left[x^k-\gamma \nabla f(x^k)\right]_{\mathcal{X}}$$
%  
%   communicate
% 
% The full gradient communication consists in algorithms
%
 The full gradient communication algorithms %consists in algorithms that 
  solve problems on the form  
 \begin{align}\label{eqn:Problem}
\mathop\text{minimize}\limits_{x\in X} \quad f(x), %= \sum_{i=1}^n f_i(x),
\end{align}
 by performing a standard (projected) gradient method
 $$x^{k+1}=\left[x^k-\gamma \nabla f(x^k)\right]_{\mathcal{X}}$$
  where the full gradient $ \nabla f(x^k)$ is communicated at every iteration.
 Such communication appears in dual decomposition methods where $f(\cdot)$ is a dual function associated with some large-scale primal problem, we illustrate this  in Subsection~\ref{sec:Mot_Dist1}. 
 The partial gradient communication algorithms   %consists in algorithms for
 solve separable optimization problems between $n$ nodes  on the form
 \begin{align}\label{eqn:Problem}
\mathop\text{minimize}\limits_{x} \quad f(x) = \sum_{i=1}^n f_i(x),
\end{align}
 %
%
 %
 %
  by  performing a separable gradient method
  $$x^{k+1}=x^k-\gamma \sum_{i=1}^n \nabla f_i(x^k)$$
   where the partial gradient $\nabla f_i(x^k)$ is communicated by node  $i$, see Subsection~\ref{subsec:PartialGradient}. % needs to communicates its gradient $\nabla f_i(x^k)$. 
  Clearly, the the full gradient communication is a special case of the partial gradient communication with $n=1$.  
  However, considering the full gradient communication algorithms separately  will enable us to get stronger results in that case. We now review these algorithms separately in the next subsections.
  %
%  a) Full gradient communication architecture where the full gradient $\nabla f(x)$ is communicated at every iteration and b) partial  gradient communication architecture where 
% $$f(x)=\sum_{i=1}^n f_i(x),$$
% .  We review these two communication architectures, respectively, in the next two subsections. 
}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%% OLD TEXTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% OLD TEXTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% OLD TEXTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% OLD TEXTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


















\begin{figure}[t]%htb]
    \centering % <-- added
\begin{subfigure}{0.5\textwidth}
\centering
  \includegraphics[scale=0.5]{Introduction/Figures_inkscape_ICCOPT/FullGradientArchitecture}
  %/home/sarit/Documents/Papers/Papers/2018/Sindri/Figures_inkscape/full_gradientCommunication}
  \caption{}
  \label{fig:centralized}
\end{subfigure}\hfill % <-- added
\begin{subfigure}{0.5\textwidth}\centering
  \includegraphics[scale=0.5]{Introduction/Figures_inkscape_ICCOPT/PartialGradientArchitecture}
  %{/home/sarit/Documents/Papers/Papers/2018/Sindri/Figures_inkscape/drawing}
  \caption{}
  \label{fig:distributed}
\end{subfigure}
\caption{Two common communication architectures for distributed gradient methods: 1) full gradient communication (left)  and 2) partial gradient communication (right).  
%\Sindri{For figure 1a, it is maybe more natural to change the text "central node" to "Users" and "worker node" to "sources", so the better math the application examples in Section 3.1.1.. Also maybe it would be more clear to include the gradients in the figure, then $\nabla f(x)$ in figure 1a and $\nabla f_i(x)$ in figure 1.b.  There also needs to be some reference and explaining of the figures in Sections 3.1.1 and 3.1.2. }
}
\label{fig:distributedlearningframework}
\end{figure}



\subsubsection{Full Gradient Communication: Dual Decomposition} \label{sec:Mot_Dist1}


%\Sindri{To be consistent with the partial gradient communication and the results, we need to include gradient noise.  This is is natural when doing dual decomposition, the dual gradients often comes from measurements, I can include some references on this later.}

\emph{Resource allocation} is the modern distributed optimization problem where a group of $p$ %\footnote{\Sindri{Consider using other notation than $n$ here to avoid confusing with the partial gradient.}} 
nodes aim to minimize the sum of their local utility function over coupled/shared constraints (\emph{e.g.}, resource limitations). In particular, all nodes collaboratively solve 
%\Sindri{In this optimizaton problem we use the notation $g()$, I changed it to $h()$  so it is not confused with the stochastic gradient)}
%\Sindri{We could make this problem be a equality constrained problem, then we get an unconstrained dual problem.}
\begin{equation} \label{EQ:ProblemFullGradient}
\begin{aligned}
& \underset{q_1,\ldots,q_n}{\text{minimize}}
& & \sum_{i=1}^n U_i(q_i)\\
& \text{subject to}
& & h(q_1,q_2,\ldots,q_n) =  0, \\  %~~(\text{or } g(q_1,\ldots,q_N )\leq 0)\\
&&& q_i\in \mathcal{Q}_i,~~i=1,\ldots,n.
\end{aligned}
\end{equation}
Here, each node has its private decision variable $q_i$ with associated utility function $U_i(q_i)$ and the constraint set $\mathcal{Q}_i$. The decision variables are coupled through the constraint $h(q_1,q_2,\ldots,q_n) =  0$, which captures physical or economical limitations. 

Resource allocation problems often arise in wireless networks, data communications, and smart grids, \cite{li2011optimal,madan2006distributed,low1999optimization}. In data communications we optimize the data flows
 between $n$ destination pairs through an $L-$link communications network by  solving the utility minimization problem~\eqref{EQ:ProblemFullGradient} with $h(q_1,q_2,\ldots,q_n)=\sum_{s\in \mathcal{S}_l} q_s - c_l$ for $l\in[1,L]$ and  $\mathcal{Q}_i=  [\underline{q}_i,\bar{q}_i]$ for $i\in[1,n]$, \cite{low1999optimization}. 
 %
 %
 %
 %
 \iffalse
 solving the following utility minimization problem \cite{low1999optimization}
 \Sindri{Probably we can explain network flow problems in words to save space. This is a good place to compress if we need to do that.}
%
 \begin{equation} \label{EQ:TCP}
\begin{aligned}
& \underset{q_1,\ldots,q_n\in \mathbb{R}}{\text{minimize}} & & \sum_{i=1}^n U_i(q_i)\\
& \text{subject to} & & \sum_{s\in \mathcal{S}_l} q_s \leq c_l, ~~~l=1,\ldots,L\\  %~~(\text{or } g(q_1,\ldots,q_N )\leq 0)\\
& & & q_i\in [\underline{q}_i,\bar{q}_i]~~i=1,\ldots,n.
\end{aligned}
\end{equation}
\fi
Here,  $\mathcal{S}_l$ is a set containing the source/destination pairs that use link $l$, and $U_i(\cdot)$ represents data utility to or priority of each user.
%or fairness or priority between the different source/destination pairs when allocating the data. 
%  Similarly, in wireless networks, we can optimize data-rates while using shared  there the coupling constraints  optimize  utilities and constraints further model collations package-drop 
 In electric power systems problems on the form of~\eqref{EQ:ProblemFullGradient} are used to optimize the electricity generation and consumptions of a group of electric devices (\emph{e.g.}, smart meters, household appliances and renewable generators)  where $h(q_1,q_2,\ldots,q_n)= 0$ represents the physics of the grid.
 
The solution to problems on this form is typically decomposed by considering the dual problem,~\cite{low1999optimization,chiang2007layering,palomar2006tutorial,zhao2014design,magnusson2017convergence,magnusson2016distributed}. To illustrate this procedure, we consider the following dual problem which is equivalent to solving \eqref{EQ:ProblemFullGradient} (under mild technical conditions~\cite[chapter 5]{boyd2004convex})
\begin{equation} \label{EQ:ProblemFullDual}
\begin{aligned}
 & \underset{x}{\text{maximize}}
& & f(x):= \min_{q} L(q,x), %\\
%&&& \lambda \geq 0
\end{aligned}
\end{equation}
 where  $x$ is the dual variable, $f(x)$ is the dual objective function,  and  %is the given by
% To construct the dual problem we consider the Lagrangian function
$$L(q,x)= \sum_{i=1}^n U_i(q_i)+x^T h(q_1,\ldots,q_n ),$$
is the Lagrangian of Problem~\eqref{EQ:ProblemFullGradient}.
%where  $\lambda$ is the dual variable.  The dual function  % is
%$$ D(\lambda)= \min_{q} L(q,\lambda)$$
 The dual function is concave and the dual gradient (or a dual subgradient) is given by
 $$\nabla f(x)= h(q_1(x),\ldots,q_n(x) ),~~~~q(x)=\underset{q}{\text{argmin}}\, L(q,x).$$
 In many networks the dual gradient is obtained from measurements based on the nodes' decisions (or inputs). Typically, we only access to a stochastic version of the gradient denoted by $g(x, \xi)$ where $\xi$ is a random variable. 
 If the primal problem has a certain structure, then dual gradient methods can often be used to decompose its solution. 
 For example, in many network applications  $h(q_1(x),\ldots,q_n(x) ) = \sum_{i=1}^n h_i(q_1(x),\ldots,q_n(x))$. Then, the equivalent dual problem \eqref{EQ:ProblemFullDual} can be solved by the projected gradient method \eqref{eqn:FullGDcentralized} which forms the following iteration:
 \begin{align*}
         q_i^{k+1}=&\underset{q}{\text{argmin}} ~U_i(q_i^k) +(x^k)^T  h_i(q_i^k) , ~~~~i=1,\ldots,n \\
        x^{k+1} =& x^k + \gamma g(x^k;\xi^k)
        % x^{k+1} =& \left\lceil x^k+\gamma \nabla g(x^k, \xi^k) \right\rceil_+ 
        % g(q_1^{k+1},\ldots,q_n^{k+1} )\right\rceil_+
 \end{align*}
 where $\gamma$ is the fixed, positive step-size.  % If performing the optimization in computing $q^{k+1}$ is difficult then we might consider taking a gradient step also for the primal variable:
% \begin{align*}
%         q_i^{k+1}=& q^{k} - \gamma\left( \nabla U_i(q_i) +\sum_{i=1}^n \lambda_i^k  \nabla g_i(q_i^k) \right) , ~~i=1,\ldots,n
%       \\%=& \left\lceil \lambda^k+\gamma \nabla D(\lambda^k) \right\rceil_+ 
%       \lambda^{k+1} =&  \left\lceil \lambda^k+\gamma 
%         g(q_1^{k+1},\ldots,q_n^{k+1} )\right\rceil_+ .
% \end{align*}
Notice that the essential step in the algorithm is the communication of the stochastic dual gradient $g(x^k, \xi^k)\approx h(q_1^{k+1},\ldots,q_n^{k+1})$ which allows the node to update $q_i^{k+1}$ based only on the  dual variable $x^k$. {To communicate the gradient it must first be compressed into the finite number of bits. Our results in this paper illustrate how to improve naive, direct gradient compression by an error correction step which in turn leads to significant solution accuracy improvements. }
% must be compressed before goal of this work  this paper we illustrate how to compress the communication gradient }
%
%

% Problem~\eqref{EQ:TCP} 
 
%\SM{We have just discussed an instances of Problem~\eqref{eqn:Problem} where the local objective functions were coupled with a shared constraints.  However, in many applications the coupling is in the objective function, we discuss such problems next. }
% are no coupling constraints but the coupling betweenthat the local  next another very common setting of distributed optimziation

\subsubsection{Partial Gradient Communication} \label{subsec:PartialGradient}


%\Sindri{We could introduce  Problem~\eqref{eqn:Problem} in this subsection. In the initial paragraph of  Section~\ref{sec:Mot_Dist} we should either include a more general problem that covers both Problem~\eqref{eqn:Problem} and the constrained problem in Equation~\eqref{EQ:ProblemFullGradient} or skip giving a mathematical formulation.  It is strange to see here: now we consider the problem we defined long time a go and have not discussed since then.    }
%\Sindri{This discussion needs to a bit general, now it feels like our work only covers empirical risk minimization. But it covers any problem on the form of~\eqref{eqn:Problem} where there is operator coordinating local objective functions.  }

%\Sindri{I feel that we go quickly to ERM. We want people to realize that this is a general problem, ERM is just one application.  I  added 1-2 sentences before the ERM discussion. }

%\Sindri{There are some issues with Problem~\eqref{eqn:fi_ERM} and the discussion of the ERM.  $m$ and $n$ are sometimes mixed up, first sentence: m nodes, later agent $i\in [1,n]$. $1/m$ should be $1/(nm)$, divid by total number of data points.}


Another setting of distributed optimization is where $n$ nodes wish to solve the separable problem \eqref{eqn:Problem}. 
%
%the sum of local objective functions as follows:
%In this paper,  we consider the minimization problem over the average of a large number of smooth, differentiable functions
%\begin{align}\label{eqn:Problem}
  %  \mathop{ \text{minimize}}\limits_{x\in\mathbb{R}^d} \quad f(x) = \frac{1}{m}\sum_{i=1}^m f_i(x).
%\end{align}
%
%
%Problem \eqref{eqn:Problem}, also known as \emph{empirical risk minimization} (ERM), arises in machine learning, statistics and signal processing. This problem includes least-squares estimation, logistic regression, and support vector machines.
%Here the objective function $f_i(x)$ is maintained locally by node $i$
Here, the goal is to determine the common decision variable $x$ based on the local objective functions $f_i$ kept by each node $i$. Problems on this form commonly appear in machine learning and signal processing where we wish to find  optimal estimators based on data from multiple nodes. Common optimization problems appearing in these applications are \emph{empirical risk minimization} (ERM), where labelled data is split among the $n$ nodes, which collaboratively find optimal estimators. In particular,  if each node $i\in [1,n]$ has access to its local data with feature vectors $\vec{z}_i=(z_i^1,\ldots,z_i^m)$ and labels $\vec{y}_i=(y_i^1,\ldots,y_i^m)$ with $z_i^j\in \mathbb{R}^d$ and $ y_i^j\in \mathbb{R}$, then the local objective functions  have the form
%
%
\begin{align}\label{eqn:fi_ERM}
f_i(x)=\frac{1}{m}\sum_{j=1}^m \ell(x; z_i^j,y_i^j)+ \frac{\lambda}{2}||x||^2, \quad \text{for } i=1,2,\ldots,n
\end{align}
%
%
where $\ell(\cdot)$ are some loss functions and $\lambda>0$ is the regularization parameter. This optimization problem covers many important machine learning approaches. For example, we obtain the least-squares regression problem if $\ell(x; z,y)=  (1/2)(y- z^T x)^2$, the logistic regression problem if $\ell(x; z,y)=\log(1+\exp(-y\cdot z^T x)),$ and the  Support Vector Machines (SVMs) problem if  $\ell(x; z,y)= \left\lceil1-y\cdot z^T x \right\rceil_+.$


%\Sindri{Lets try to get to the main message as quickly as possible.  \textbf{Main Message}: This problem is typically solved in a distributed fashion by having each node compute local gradient and communicate it to the master. \textbf{Secondary message}: When there are many data points then we can do stochastic gradient or mini-batch, our results cover this cases as well. Now the \textbf{Main Message} is hidden in a long discussion on the \textbf{Secondary Message}. People will easily miss the main point that the gradients are communicated and need to be compressed. So it is better if we first make the \textbf{Main Message} clear and then discuss the \textbf{Secondary Message}.    }



When the data-set on each node is large, then the above optimization problem is typically solved with stochastic gradient decent methods (SGD).
%
%
%
%
%{For data-intensive applications,  distributed stochastic gradient descent (SGD) is among the common randomized first-order algorithms due to near-optimal iteration complexity by proper step-size tuning~\cite{needell2014stochastic}, and easy utilization in massive parallelization by multiple nodes in a computer cluster.}
%
%
 In each iteration of distributed SGD, the master node broadcasts a decision variable $x^k$, while each worker node $i$ queries a stochastic gradient 
$\nabla g_i(x^k;\xi_i^k)$ with the random index $\xi_i^k$ selecting part of its local data $\mathcal{D}_i$. After the master  receives the information from all worker nodes, it can perform the update
%
%
% 
\begin{align}\label{eqn:minibatchSGD}
x^{k+1}=x^k-\gamma \frac{1}{n}\sum_{i=1}^n g_i(x^k;\xi_i^k).
\end{align}
Here, the stochastic gradient preserves unbiased property, i.e. 
\begin{align}\label{eqn:unbiasednessSGD}
\mathbb{E}_{\xi_i}  g_i(x;\xi_i) = \nabla f_i(x), \quad \forall x\in\mathbb{R}^d
\end{align}
and satisfies the bounded variance assumption, i.e. 
\begin{align}\label{eqn:boundedvarianceSGD}
\mathbb{E}_{\xi_i} \|  g_i(x;\xi_i) - \nabla f_i(x) \|^2 \leq \sigma^2, \quad \forall x\in\mathbb{R}^d. 
\end{align}
Notice that unlike \cite[Assumption 1]{lian2015asynchronous} and
\cite[Assumption 3]{feyzmahdavian2016asynchronous} this bounded variance assumption only imposes similarity between the local gradient and its stochastic oracle, which allows for arbitrary difference between the whole data and local data  distributions. For the $\ell_2-$regularized ERM, $\nabla g_i(x;\xi_i) = (1/|\mathcal{B}_i|)\sum_{j\in \mathcal{B}_i}\nabla \ell(x;z_i^j,y_i^j) + \lambda x,$ where the mini-batch $\mathcal{B}_i$ is the subset of data $\mathcal{D}_i$ of size $|\mathcal{B}_i|$ at worker node $i$, which is selected uniformly at random. %Also, the associated Hessian information of the stochastic gradient for the $\ell_2-$regularized ERM becomes $\nabla^2 g_i(x;\xi_i) =  (1/|\mathcal{B}_i|)\sum_{j\in \mathcal{B}_i}\nabla^2 \ell(x;z_i^j,y_i^j) + \lambda I$.
Clearly, distributed gradient descent \eqref{eqn:fulldistGD} is a special case of distributed SGD \eqref{eqn:minibatchSGD} with $\nabla g_i(x;\xi_i) = \nabla f_i(x)$. 




To save communications bandwidth, worker nodes need to compress gradients into low-precision representation. To show our results which illustrate benefits of error compensation on distributed SGD with gradient compression, we now present the compression schemes considered in this paper. 

 
 

\iffalse
\emph{stochastic gradient descent} (SGD) is among the most popular randomized first-order algorithms, since it enjoys a low per-iteration cost and small memory footprints, \cite{needell2014stochastic}.

For unprecedented huge-scale data sets in modern engineering applications, \emph{stochastic gradient descent} (SGD) is among the most popular randomized first-order algorithms, since it enjoys a low per-iteration cost and small memory footprints, \cite{needell2014stochastic}. Even though theoretically and empirically proven to have near-optimal iteration complexity by proper step-size tuning \cite{needell2014stochastic}, SGD has severely limited performance scalability by its  inherently sequential computation. 

One simple modification is \emph{mini-batching}, which processes several samples per iteration and allows to reduce the variance of gradient estimates. Mini-batch SGD takes smaller iteration counts and enjoys significantly low training time, since it can easily utilize massive parallelization to attain high scalability by modern multi-core processors, or even by computer clusters. In each iteration of mini-batch SGD under distributed frameworks, the master node typically broadcasts a decision variable $x^k$, while each worker node $i$ queries a stochastic gradient 
$\nabla g_i(x^k;\xi_i^k)$ with the random index $\xi_i^k$ selecting part of its local data $\mathcal{D}_i$. After the master  receives the information from all worker nodes, it can perform the update
%
%
% 
\begin{align}\label{eqn:minibatchSGD}
x^{k+1}=x^k-\gamma \frac{1}{n}\sum_{i=1}^n \nabla g_i(x^k;\xi_i^k).
\end{align}
Here, the stochastic gradient preserves unbiased property, i.e. 
\begin{align}
\mathbb{E}_{\xi_i} \nabla g_i(x;\xi_i) = \nabla f_i(x), \quad \forall x\in\mathbb{R}^d.
\end{align}
For the $\ell_2-$regularized ERM, $\nabla g_i(x;\xi_i) = (1/|\mathcal{B}_i|)\sum_{j\in \mathcal{B}_i}\nabla \ell(x;z_i^j,y_i^j) + \lambda x,$ where the mini-batch $\mathcal{B}_i$ is the subset of data $\mathcal{D}_i$ of size $|\mathcal{B}_i|$ at worker node $i$, which is selected uniformly at random. Also, the associated Hessian information of the stochastic gradient for the $\ell_2-$regularized ERM becomes $\nabla^2 g_i(x;\xi_i) =  (1/|\mathcal{B}_i|)\sum_{j\in \mathcal{B}_i}\nabla^2 \ell(x;z_i^j,y_i^j) + \lambda I$.
\fi
%
%
%Even though many works proved the convergence rate of distributed mini-batch SGD \cite{lian2017can,lian2015asynchronous,feyzmahdavian2016asynchronous,alistarh2017qsgd}, they assume similarity between local data distributions $\mathcal{D}_i$ and the whole data distribution $\cup_{i=1}^m \mathcal{D}_i$. The results imply significantly slow convergence of distributed mini-batch SGD even with low solution accuracy since the cluster in practice contains computer nodes with too different computing performance and memory requirements.  Following \cite{mishchenko2019distributed}, our analysis admits highly heterogeneous data distributions among the worker nodes. 
%
%





%
%accomplish these distributed algorithms some communication is needed, which generally requires some %compression or distortion of the communication gradients. 




 



\iffalse
For large-scale datasets, Problem~\eqref{eqn:Problem} is solved in a distributed manner where a master node coordinates the executation of a first-order method, typically gradient descent or stochastic gradient descent. 
To that end, the master node typically broadcasts a decision variable $x^k$ at each iteration, while
each node  $i$ communicates back either the gradient $\nabla f_i(x^k)$ based on the full local data at node $i$ or a stochastic gradient based on part of the data (a mini-batch) at node $i$. 
\fi

\iffalse
To limit the amount of data exchanged in these distributed algorithms, it has been suggested to compress or quantize the gradients before they are communicated. 
%accomplish these distributed algorithms some communication is needed, which generally requires some %compression or distortion of the communication gradients. 
We now review the compression schemes we consider in this paper. 
\fi























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    Gradient Compression
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Gradient Compression} \label{sec:Mot_GC}
%This section introduces two families of generic compression operators.

%\Sindri{Remove first two sentences. We should motivate this well in the introduction, but we don't need to keep recalling it. It easily gets tiring.  Lets get quickly to the main point. Before going to definition 1, we need to make the following message clear: Our results work for very general class gradient compressions, that is all compressions satisfying Defintion 1.
%}


To study effects of error compensation mechanisms on compressed gradient methods, we consider general compressors having the following property.




%\replaced{}{Under distributed learning frameworks, communication costs of the exchange of gradient vectors among computer nodes within a cluster can easily lead to significant performance limitations especially for problems with huge dimension. One common way is to compress the gradient vector before broadcasting it into a finite precision which can be represented by a few numbers of communicated bits. }
%
%
%
\iffalse
In practice we need to compress the gradient vectors to finite precision before we can communicate them. % communication  it generally needs to be compressed.  
 For example, to implement the  full gradient methods in Subsection~\ref{sec:Mot_Dist1}  we need to compress the gradient $\nabla f(x)$, resulting in the compressed gradient method % version of the gradient $\nabla f(x)$, instead of the gradient itself. 
 \begin{equation} \label{eq:CompressedGradient} 
    x^{k+1}=x^k-\gamma Q(\nabla f(x^k))
 \end{equation}
  where $Q(\nabla f(x^k))$ is a compression operator that maps the gradient to finite precision.  More agressive  compression  leads to smaller data exchange but also lower precision.
 \fi 
%  
% 
% do note communicate the gradient $\nabla f(x)$ itself, but instead we co is communicated we compressed it with some
%
%\replaced{
%The main goal of this paper is to study error-compensation schemes for compressed gradient methods. 
%Our results apply for very general class gradient compressions, i.e., any compression operator that satisfies the following definition.}{In this paper, we study a wide range of compression schemes and an  error-compensation mechanism that work well on all of them.  In particular, we consider both deterministic and stochastic compression operations defined as follows.}
%
%
%
%
\begin{definition}\label{def:DBEC} %\footnote{\Sindri{I cannot see any stochastic compressors. So it is best to not say deterministic.  We consider $\epsilon$-compressor, otherwise the reviewers will probably ask about stochastic gradients and comparison. }}
The operator $Q:\mathbb{R}^d\rightarrow\mathbb{R}^d$ is an $\epsilon-$\emph{compressor} if there exists a positive constant $\epsilon$ such that
\begin{align*}
\| Q(v) - v \| \leq \epsilon, \quad \forall v\in\mathbb{R}^d.
\end{align*}
\end{definition}




%\Sindri{We should first have few sentences discussing the intuition of the definition, what does it mean? what does it imply? Then we can compare it to others.}

From Definition \ref{def:DBEC} we require only the bounded magnitude of quantization error, which  implies high compression accuracy if $\epsilon$ has low value (e.g. $Q(v)=v$ when $\epsilon=0$). The compressors according to Definition \ref{def:DBEC} are not require to be unbiased  unlike \cite{alistarh2017qsgd,khirirat2018distributed}, and are allowed to have  quantization error arbitrarily larger than magnitude of the original vector unlike \cite[Definition 2.1]{Stich2018} and \cite[Assumption A]{2019arXiv190109847P}. Definition \ref{def:DBEC} covers popular compressors in machine learning and signal processing appplications, which substantiates the generality of our results later in the paper. 
%
%
%
One common example is a rounding quantizer, where  each element of a full-precision vector $v_i\in\mathbb{R}$ is rounded to the closet point in a grid with  resolution level $\Delta>0$ according to 
\begin{align}\label{eqn:RoundingQuant}
[Q_{dr}(v)]_i &= {\rm sign}(v_i) \cdot \Delta\cdot \floor*{ \frac{|v_i|}{\Delta} +\frac{1}{2}}.
\end{align}
%
%
%
\iffalse
%{\color{red} \textbf{Sindri:} I prefer not to have the examples of compressions as definitions, it makes the message
\Sindri{maybe to formal to have this quantizator as an Example. Could  presented as a numbered equation, if we are referring to it later.}
\begin{example}[\cite{li2017training,rabbat2005quantized,zhu2016quantized}]\label{def:deterRQ}
For a given quantization resolution $\Delta >0$, the \emph{rounding quantizer} $Q_{dr}:\mathbb{R}^d\rightarrow\Lambda$ is defined as
\begin{align*}
[Q_{dr}(v)]_i &= {\rm sign}(v_i) \cdot \Delta\cdot \floor*{ \frac{|v_i|}{\Delta} +\frac{1}{2}}, 
\end{align*}
where $v\in\mathbb{R}^d$.
\end{example}
\fi
%
%
%
This rounding quantizer  is a  $\epsilon-$compressor with $\epsilon = d\cdot\Delta^2/4$, \cite{rabbat2005quantized,zhu2016quantized,li2017training,de2018high}. 
%
%
In addition, if we assume bounded gradient assumptions and apply the compressor on gradients, then the sign compressor \cite{seide20141}, the $K-$greedy quantizer \cite{gradientcompression2018} and the dynamic gradient quantizer \cite{alistarh2017qsgd,gradientcompression2018} all are $\epsilon$- compressors.



% some sentences saying that making the bounded gradient assumptions implies definitions of our compressors include these results. 

%\begin{itemize}
%	\item Perhaps mention something about other quantizers under bounded gradient assumption?
%\end{itemize}



















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Direct Gradient Compression: Lower Bounds and Convergence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{The Limits of Direct Gradient Compression} %: Lower Bounds and Convergence}
\label{sec:Mot_Low}
%\begin{itemize}
%	\item Add some introductory glue text here\dots 
%\end{itemize}
%\Sindri{See my comment in the beginning of the paper, probably best to let this be a separate section. The comment I have written here, address them last. We first need to structure this section.   
%Let's not do anything with this section for the moment, let's first fix the other sections.  I think we should move all  discussion on Direct Gradient Compression here, see my comment below. This will probably need to be a separate Section, we will also probably need to rethink a bit the structure.}

%\Sindri{This first sentence is very long and complicated, it needs to be split into few of simpler sentences.   
 %Think about the main message.  I would start by saying something like this:
  % }
 %\Sindri{It feels natural to have this as a separate section. Also, like I said also in my last bunch of comments: We need to improve the flow here and make this section a bit more structured. I think it is most natural to splitting this section up into 3 subsections in the following order 1) Full Gradient Communication 2) Partial Gradient Communication 3) Limits of Direct Compression: Lower Bound.  We need to be were clear on the message from the beginning: \emph{The most straightforward approach is to directly compress the gradients, this section shows the limit of this approach.}     }


To save the number of communicated bits in distributed optimization, it is most straightforward to compress the gradients directly.  The goal of this section is to illustrate the limits of this approach, which motivates our gradient correction compression algorithms in the next section.


\subsection{Full Gradient Communication}

We start by studying direct compression under full gradient communication architecture. In particular, we consider compressed stochastic gradient descent algorithm (CSGD)
which queries the stochastic gradient $\nabla g(x^k;\xi^k)$ and updates the iterate according to the following iteration:
%In the distributed optimization algorithms, gradient information is compressed in each iteration. Many works suggest that communications using low-precision gradients    may save communicated bits, but often suffer from extremely low solution accuracy. In this section, we show that this intuition is correct for naive, direct gradient compression. However, we later show how to obtain arbitrarily high solution accuracy with low-precision gradient information by using error compensation.  Now, we show the limits of direct gradient compression by considering full gradient communication architecture in Section~\ref{sec:Mot_Dist1}. In particular, we study compressed gradient descent (CGD) which forms the following iteration: given the fixed positive step-size $\gamma$, and the initial point $x^0\in\mathbb{R}^d$
%
%
\begin{align}\label{eqn:CGD}
x^{k+1} = x^k - \gamma Q\left( \nabla g(x^k;\xi^k) \right),
\end{align}
where  the stochastic gradient  $\nabla g(x;\xi)$ satisfies the unbiased property and the bounded variance assumption, i.e.
\begin{align}\label{eqn:UnbiasedBoundedVariance_full}
\mathbb{E}_{\xi}  \nabla g(x;\xi) = \nabla f(x) \quad \text{and} \quad \mathbb{E}_{\xi}\| \nabla g(x;\xi)  - \nabla f(x) \|^2 \leq \sigma^2, \quad \forall x\in\mathbb{R}^d.
\end{align}
%
%
%
%
Note that CSGD with $\nabla g(x^k;\xi^k) = \nabla f(x^k)$ recovers standard gradient descent which is commonly applied on the dual function in dual decomposition under the full gradient communication architecture (see  Section~\ref{sec:Mot_Dist1}).



Before providing CSGD convergence, we begin by showing the direct gradient compression in~\eqref{eqn:CGD} degrades solution accuracy since it accumulates error at every iteration. This can be seen by considering the case where there is no gradient noise,  $\nabla g(x^k;\xi^k) = \nabla f(x^k)$, and where the objective function is quadratic, 
\begin{align} \label{eq:quadOBJ}
     f(x)=\frac{1}{2}x^T Hx + b^Tx. 
\end{align}
In this case the CSGD update in~\eqref{eqn:CGD} can be reduced to 
\begin{align} \label{eq:xupdate}
   x^{k+1} =& \overbrace{(I-\gamma H)}^{:=A_{\gamma}}x^k -\gamma b+\gamma \left( \nabla f(x^k)-Q\left(\nabla f(x^k) \right) \right),
\end{align}
which yields 
$$ x^{k+1}-x^{\star}= A_{\gamma}^{k+1}(x^0-x^{\star})+\gamma \sum_{j=0}^k A_{\gamma}^{k-j} \left( \nabla f(x^j)-Q\left(\nabla f(x^j) \right) \right)  $$
where $x^{\star}$ is the optimal solution and we used the fact that $H x^\star + b=0$. Notice that direct compression accumulates quantization errors as seen in the final term. We show later that error compensation helps remove this accumulation as presented in Section~\ref{sec:ECGC}. Even though the error accumulates, the compression error will remain bounded if the matrix $A_{\gamma}$ is stable, as illustrated in the following theorem. 
%
%Our first result characterizes  the linear  convergence rate of CSGD with $\nabla g(x^k;\xi^k) = \nabla f(x^k)$  and $\omega^k = 0$ for strongly convex quadratic optimization. 
 %
 %
 

\begin{theorem} \label{thm:CGDQuadratic}
Consider the quadratic optimization problem over the objective function~\eqref{eq:quadOBJ} where $H$ is positive definite and let $\mu$ and $L$ be the smallest and largest eigenvalues of $H$, respectively. Then, the iterates $\{x^k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:CGD} with $\nabla g(x^k;\xi^k) = \nabla f(x^k)$satisfy
\begin{align*}
\| x^k - x^\star \| &\leq \rho^k\| x^0 - x^\star \| + \frac{1}{\mu}\epsilon, 
\end{align*}
where
\begin{align*}
\rho &= \left\{ \begin{array}{ll} 1-1/\kappa & \text{if } \quad \gamma = 1/L \\   1-{2}/{(\kappa+1)} & \text{if }\quad \gamma = 2/(\mu+L)   \end{array}\right.  ,
\end{align*}
and $\kappa = L/\mu$ is the condition number of $H$.
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:CGDQuadratic}.
\end{proof}
%
%Theorem \ref{thm:CGDQuadratic} establishes the linear convergence rate of CGD~\eqref{eqn:CGD} for strongly convex quadratic optimization. Note that if the whole objective function $f(x)=(1/2)x^2$, then the lower bound matches the upper bound by Theorem \ref{thm:CGDQuadratic}.
% 
Theorem \ref{thm:CGDQuadratic} shows that  compressed gradient descent in Equation~\eqref{eqn:CGD} converges linearly toward solution with residual error $\epsilon/\mu$ where $\epsilon$ is the quantization error and $\mu$ is the smallest eigenvalue of $H$ (or the strong convexity parameter of the  quadratic objective function). We illustrate in Section~\ref{subsec:Limits} that the upper bound in the theorem is tight.  With our error-compensated method as presented in Section~\ref{sec:ECGC} we can achieve arbitrarily high solution accuracy even for fixed $\epsilon>0$ and $\mu>0$. Similar results as presented in Theorem~\ref{thm:CGDQuadratic} can be obtained for general objective functions and with stochastic gradients in Section~\ref{subsec:CpartialGradient}.


\iffalse
\sarit{remove this theorem and move discussions to theorems for partial gradient communication}

%To show that the above lower bound is tight, we provide the worst-case upper bound of the convergence rate of CGD~\eqref{eqn:CGD} in the following theorem.
\begin{theorem}\label{thm:CGDimproved} 
Consider an optimization problem \eqref{eqn:Problem} and the iterates $\{x^k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:CGD}. Assume that we choose the $\epsilon-$compressor, and $\gamma < 1/(4L)$. If the whole objective function $f$ is $L-$smooth, then  
\begin{align} \label{eq:ThmFull1}
\mathop{\min}\limits_{l\in[0,k]} \mathbf{E}\| \nabla f(x^l)\|^2 
& \leq \frac{2}{\gamma}\frac{1}{1-4L\gamma}\left( f(x^0) - f(x^\star) \right) \\
&\hspace{0.4cm} + \frac{4L}{1-4 L\gamma}\gamma (\sigma^2_v + \sigma_\omega^2)+\frac{1+4L\gamma}{1-4L\gamma}\epsilon^2.
\end{align}
In addition, if $f$ is also $\mu$-strongly convex, then
\begin{align} \label{eq:ThmFull2}
\mathbf{E}\left(  f(\bar x^k) - f(x^\star) \right)  
& \leq \frac{1}{k+1}\frac{1}{4\gamma}\frac{1}{1-4L\gamma}\| x^0 - x^\star \|^2 \\
&\hspace{0.4cm} +\frac{2}{1-4L\gamma}\gamma (\sigma^2_v + \sigma^2_\omega) + \frac{1}{2}\frac{1/\mu+4\gamma}{1-4L\gamma}\epsilon^2,
\end{align}
where $\bar x^k = \sum_{l=0}^k x^l/(k+1)$.
\end{theorem}
\begin{proof}
See Appendix \ref{app:CGD}.
\end{proof}
%
% \Sindri{We need to explain in words the implication of the theorem.  } 
% \SM{ The above theorem gives a convergence rate results on the CGD method in Equation~\eqref{eqn:CGD}. In particular, it shows that when...   We use this result as a reference }
 %
 %
 
 
Theorem \ref{thm:CGDimproved} establishes a sub-linear convergence rate of CSGD \replaced{to an approximate solution whose accuracy depends on $\epsilon$, $\gamma$, $\mu$, $L$, and the gradient noise.}{}. 
 
\replaced{The solution accuracy in both equation~\eqref{eq:ThmFull1} and~\eqref{eq:ThmFull2} has two terms. The first term comes from the gradient noise. This  term will go to zero as the step-size $\gamma$ is decreased.  
The second term comes from the quantization and depends on the quanization level $\epsilon$.  This term cannot be decreased to zero with diminishing step-size $\gamma$.  In fact, it can be bounded by noting that
$$\frac{1+4L\gamma}{1-4L\gamma}>1 ~~~\text{and}~~~ \frac{1}{2}\frac{1/\mu+4\gamma}{1-4L\gamma}>\frac{1}{2\mu}, $$
for $\gamma\in (0,1/(4L))$.
This means that the upper bound in Equation~\eqref{eq:ThmFull1} cannot become smaller than $\epsilon^2$ and the  upper bound in Equation~\eqref{eq:ThmFull2} cannot become smaller than $\epsilon^2/(2\mu)$. 
 We give an example in Section~\ref{subsec:Limits} where this upper bound is tight.
}{
 Notice that solution accuracy depends on the stochastic gradient, the stochastic noise and the resolution level of quantization. In particular, low step-size $\gamma$ leads to slow convergence but high solution accuracy. } 


\Sindri{I included the discussion below in the text above.}
\replaced{}{
Next, we show direct compression cannot attain solution accuracy lower than a certain threshold. Consider the case when $k\rightarrow\infty$, and $\nabla g(x;\xi)=\nabla f(x)$ and $\omega=0$ ($\sigma_v^2=\sigma_\omega^2=0$). From Theorem \ref{thm:CGDimproved}, CSGD satisfies 
%%
%%
%\begin{align*}
$\min_{l\in[0,k]} \| \nabla f(x^l) \|^2 \leq \frac{1+4L\gamma}{1-4L\gamma}\epsilon^2.$
%\end{align*}
Since ${(1+4L\gamma)}/{(1-4L\gamma)} > 1$, the lower bound $\| \nabla f(x^k) \|^2\geq \epsilon^2$ is shown to be tight in Example \ref{ex:SimpleQ}. Despite sub-linear convergence rate, CSGD hence cannot achieve solution accuracy lower than $\epsilon^2$.} 
\fi





\subsection{Partial Gradient Communication} \label{subsec:CpartialGradient}
%
In this section, we consider the direct gradient compression for partial gradient communication architecture by considering the distributed compressed stochastic gradient descent algorithm (D-CSGD)
%
%
\begin{align}\label{eqn:QDGD}
x^{k+1} = x^k - \gamma \frac{1}{n}\sum_{i=1}^n Q(\nabla g_i(x^k;\xi_i^k) ),
\end{align}
where each $\nabla g_i(x;\xi_i)$ is the partial gradient sent by worker node $i$ to the central node which satisfies the unbiased property~\eqref{eqn:unbiasednessSGD}  and the bounded variance assumption~\eqref{eqn:boundedvarianceSGD}.
\iffalse
\begin{align}\label{eqn:UnbiasedBoundedVariance_dist}
\mathbb{E}_{\xi_i}  \nabla g_i(x;\xi_i) = \nabla f_i(x) \quad \text{and} \quad \mathbb{E}_{\xi_i}\| \nabla g_i(x;\xi_i)  - \nabla f_i(x) \|^2 \leq \sigma^2, \quad \forall x\in\mathbb{R}^d.
\end{align}
\fi
%
%
We have the following convergence results which are analogous to Theorem~\ref{thm:CGDQuadratic} for full gradient communication architecture.
%
\begin{theorem}\label{thm:distCSGD_convex} 
Consider an optimization problem \eqref{eqn:Problem} and the iterates $\{x^k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:QDGD}. Assume that we choose the $\epsilon-$compressor, and $\gamma < 1/(4L)$. If the whole objective function $f$ is $L-$smooth, then  
\begin{equation}\label{eqn:distCSGD_NC}
\begin{aligned}
\mathop{\min}\limits_{l\in[0,k]} \mathbf{E}\| \nabla f(x^l)\|^2 
& \leq \frac{2}{\gamma}\frac{1}{1-4L\gamma}\left( f(x^0) - f(x^\star) \right) \\
&\hspace{0.4cm}+\frac{1+4L\gamma}{1-4L\gamma}\epsilon^2 + \frac{4L}{1-4 L\gamma}\gamma (\sigma^2_v + \sigma_\omega^2).
\end{aligned}
\end{equation}
In addition, if $f$ is also $\mu$-strongly convex, then
\begin{equation}\label{eqn:distCSGD_SC}
\begin{aligned}
\mathbf{E}\left(  f(\bar x^k) - f(x^\star) \right)  
& \leq \frac{1}{k+1}\frac{1}{4\gamma}\frac{1}{1-4L\gamma}\| x^0 - x^\star \|^2 \\
&\hspace{0.4cm}+ \frac{1}{2}\frac{1/\mu+4\gamma}{1-4L\gamma}\epsilon^2 +\frac{2}{1-4L\gamma}\gamma (\sigma^2_v + \sigma^2_\omega),
\end{aligned}
\end{equation}
where $\bar x^k = \sum_{l=0}^k x^l/(k+1)$.
\end{theorem}
\begin{proof}
See Appendix \ref{app:distCSGD}.
\end{proof}







Theorem \ref{thm:distCSGD_convex} establishes a sub-linear convergence of D-CSGD toward the optimum with residual error depending on stochastic gradient noise $\sigma$, quantization $\epsilon$, problem parameters $\mu,L$ and the step-size $\gamma.$ In particular, the residual error consists of two terms. The first one comes from the stochastic gradient noise, and decreases in  proportion to the step-size. The second term arises from the precision of quantization, and cannot diminish toward zero with diminishing step-size. In fact, it can be bounded by noting that
$$\frac{1+4L\gamma}{1-4L\gamma}>1 ~~~\text{and}~~~ \frac{1}{2}\frac{1/\mu+4\gamma}{1-4L\gamma}>\frac{1}{2\mu}, $$
for $\gamma\in (0,1/(4L))$. 
 This means that the upper bound in Equation~\eqref{eqn:distCSGD_NC} cannot become smaller than $\epsilon^2$ and the  upper bound in Equation~~\eqref{eqn:distCSGD_SC} cannot become smaller than $\epsilon^2/(2\mu)$. 
 We give an example in Section~\ref{subsec:Limits} where this upper bound is tight.









\subsection{Limits of Direct Compression: Lower Bound} \label{subsec:Limits}
%
%
In the distributed optimization algorithms, gradient information is commonly compressed in each iteration. However, many works suggest that communications using low-precision gradients may save communicated bits, but often suffer from low solution accuracy. In this section, we show that this intuition is correct for naive, direct gradient compression, and later show how to obtain arbitrarily high solution accuracy with low-precision gradient information by using error compensation.  
%
%Now, we show the limits of direct gradient compression by considering full gradient communication architecture in Section~\ref{sec:Mot_Dist1}. In particular, we study compressed gradient descent (CGD) which forms the following iteration: given the fixed positive step-size $\gamma$, and the initial point $x^0\in\mathbb{R}^d$
 %
 
To this end, we show a simple example when applying the $\epsilon-$compressor on standard gradient descent, and argue that error compensation scheme is a necessary solution.  



\iffalse
When provided quantization function $Q(\cdot)$ for compressing the communicated gradient information, 
 it is  most straightforward to directly compress the  gradient. 
%To this end, we start by studying compressed gradient descent (CGD) which forms the following iteration
%
%
 The result gradient method would be
\begin{align}\label{eqn:CGD}
x^{k+1} = x^k - \gamma Q\left( \nabla f(x^k) \right).
\end{align}
 Since we use the compressed gradient step $Q(\nabla f(x^k) )$   suggests  that we should suffer some inaccuracies in our solution.  
%  When we perform gradient methods with compressed gradients, as we did in Equation~\eqref{eq:CompressedGradient}, then intuition  suggests  that we should suffer some inaccuracies in our solution.  
  For example, if our quantizer is $\epsilon$-DBEC then we might suspect that our algorithm could only provide us with a sub-optimal solution and that the quality of the solution should be somehow related to $\epsilon$. 
  We now show that this intuition is correct  with a simple example. Will illustrate how to fix this behavior with a simple gradient correction in the next section. 
 \fi
% this h. % We illustrate of to correct for this behavior in providing our correcting scheme that fixes this behavior. 
%  
%   the gradient it is expected that we loose some information, and  such as the gradient is expected
%  
%This section studies the limitations of naive gradient compression. Under commonly-used assumptions of loss functions, gradient-based optimization algorithms converge toward the sub-optimum due to quantization noises; see \emph{e.g.}, in \cite{khirirat2018distributed}. By the simple quadratic optimization problem, we further demonstrate that simple gradient compression cannot make solution accuracy lower than a certain threshold. 


\begin{example}\label{ex:SimpleQ}
\textit{
Consider the scalar optimization problem
\begin{equation*}
\begin{aligned}
& \underset{x}{\text{minimize}}
& &  \frac{1}{2} x^2.
\end{aligned}
\end{equation*}
 Suppose that we run the compressed gradient decent algorithm with $\omega^k=0$:
 \begin{align} \label{eq:quant_gradient}
   x^{k+1}=x^k-\gamma Q(f'(x^k))=x^k-\gamma Q(x^k),
 \end{align}
 where $Q(\cdot)$ is the $\epsilon$-DBEC compression (see Definition~\ref{def:DBEC})\footnote{\textbf{Sindri:} I define $Q(\cdot)$ using $z/|z|$ rather than the $\texttt{sign}(\cdot)$ function because the generalization to higher dimension is $z-\epsilon z/||z||$ rather than $z-\epsilon \texttt{sign}(z)$.}
 $$Q(z)= \begin{cases} z-\epsilon \frac{z}{|z|} &\text{if } z\neq 0 \\ \epsilon & \text{otherwise}. \end{cases}  $$ %\texttt{sign}(z),$$
 %where $\texttt{sign}(z)=z/|z|$ if $z\neq 0$ and $\texttt{sign}(0)=1$. 
% $$|Q(z)-z|\leq \epsilon~~\text{ for all }~~ z\in \R.$$
% This condition holds for $Q(z)=z-\epsilon$ and with this $Q(\cdot)$, 
If we  take $\gamma\in (0,1]$  and $|x^0|>\epsilon$ then for all $k\in \mathbb{N}$ we have
 \begin{align*}
    |x^{k+1}-x^{\star}|=|x^{k+1}|=&|x^k-\gamma Q(f'(x^k))|\\
     %=&x^k-\gamma(x^k-\epsilon) \\
     %=&  |(1-\gamma) x^k+\gamma\epsilon |\\
     =&  (1-\gamma) |x^{k}|+\gamma\epsilon \\
     =&  (1-\gamma)^{k+1} |x^0| + \epsilon \gamma \sum_{i=0}^k (1-\gamma)^i \\
     =&  (1-\gamma)^{k+1} |x^0| + \epsilon \gamma \frac{1-(1-\gamma)^{k+1}}{\gamma} \\     
     =&  (1-\gamma)^{k+1}(|x^0|-\epsilon)+ \epsilon \\
     \geq& \epsilon,
 \end{align*}
% \begin{align*}
%    |x^{k+1}-x^{\star}|=x^{k+1}=&x^k-\gamma Q(f'(x^k))\\
%     =&x^k-\gamma(x^k-\epsilon) \\
%     =&  (1-\gamma) x^k+\gamma\epsilon \\
%     =&  (1-\gamma) x^{k}+\gamma\epsilon \\
%     =&  (1-\gamma)^{k+1} x^0 + \epsilon \gamma \sum_{i=0}^k (1-\gamma)^i \\
%     =&  (1-\gamma)^{k+1} x^0 + \epsilon \gamma \frac{1-(1-\gamma)^{k+1}}{\gamma} \\     
%     =&  (1-\gamma)^{k+1}(x^0-\epsilon)+ \epsilon \\
%     \geq& \epsilon,
% \end{align*}
 where we have used that $x^{\star}=0$. In addition, the direct consequence is $| f^\prime(x^k)|=|x^k|\geq \epsilon$ for all $k\in\mathbb{N}.$ 
 %
%
\iffalse
 By the fact that  $\gamma\in (0,1]$ and $\epsilon>0$, it is also easy to show that  for $k\in\mathbb{N}$
 \begin{align*}
 \text{\emph{sign}} \left(  x^{k+1}  \right) =   \text{\emph{sign}} \left(  x^{k}  \right).
 \end{align*}
Therefore, 
\begin{align*}
f(\bar x^k) - f(x^\star) 
& = \frac{1}{2} \left( \frac{1}{k+1}\sum_{l=0}^k x^l \right)^2 \\
& = \frac{1}{2} \frac{1}{(k+1)^2}  \left( \sum_{l=0}^k (x^l)^2 + \sum_{l=0}^k \sum_{l^\prime=0,l^\prime\neq l}^k x^l x^{l^\prime}  \right) \\
& = \frac{1}{2} \frac{1}{(k+1)^2} \left( \sum_{l=0}^k (x^l)^2 + \sum_{l=0}^k \sum_{l^\prime=0,l^\prime\neq l}^k \vert x^l \vert \cdot \vert x^{l^\prime} \vert  \right) \\
& \geq  \frac{1}{2} \epsilon^2,
\end{align*}
where we reach the last equality and the first inequality by the fact that $\text{\emph{sign}} \left(  x^{k+1}  \right) =   \text{\emph{sign}} \left(  x^{k}  \right)$, and that  $\vert x^k- x^\star\vert\geq \epsilon$ and $x^\star=0$. 
\fi
% 
% we obtain: 
 %\begin{align*}
 %\| \nabla f(x^k) \|^2 & = \vert x^k \vert^2 \geq \epsilon^2, \quad \text{and} \\ 
  %f(x^k) - f(x^\star) &= (1/2)\vert x^k \vert^2 \geq (1/2)\epsilon^2.
 %\end{align*}
 %\footnote{\textbf{Sindri:} It would be nice to also have some lower bound for the UBEC compression.}
 }

 \end{example}
 %
 %
 The above example shows that  the $\epsilon$-compressor cannot achieve better than $\epsilon$ accuracy.  However, in this paper we show the surprising fact that an arbitrarily  good accuracy can indeed be obtained even when the the gradient information compressed by this $\epsilon$-compressor if we include a simple correction step in the compressed gradient methods.
 
 






We show that the error compensation scheme indeed reaches lower-than-$\epsilon$ solution accuracy in the next section.
 
  









==> Main_Results/centralized.tex <==
\section{Error Compensated Gradient Compression}


\Sindri{The structure of this section needs to be improved.  The setup and aim also needs to be more clear. For example, it takes much effort understanding if this section is dealing with full gradient compression or partial gradient compression.  
Are we   considering directly compressing the gradient or  error compensation.  
Even in the theorem that deal with full gradient compression there is a discussion of partial objective functions $f_i(x)$, this is confusing. 
%
To start to clarify this I have suggested two main changes:
\begin{itemize}
 \item move all discussion on directly compressing the gradient $x^{k+1}=x^k-\gamma Q(\nabla f(x^k))$) to one place.  For detail, see my other comments on moving Theorem 1 and 2 to Section 2.3.
 \item better clarify the setup considered in this section, which is full gradient compression. It is good to start the section by highlighting the main objectives of the section. It helps the reader if we prepare them for what is about to come. That way people can also  see what sections are relevant to them and spend their time reading those section and maybe skip others.  We could start the section like (needs some refining):  \emph{
     This section  illustrates how we can use error compensation to improve the convergence compressed gradient methods. 
     In particular, we show how to ensure arbitrarily good solution accuracy no matter how poor the gradient compression is (for arbitrarily large $\epsilon$ in Definition 1 and 2). 
     To illustrate the main ideas,  in this section in we consider distributed gradient methods  where the \emph{full} gradient is compressed and communicated, partial gradient compressions is considered in Section~\ref{}.  }
\end{itemize} 
}



This section illustrates how to apply error compensation to improve performance from compressed gradient-based optimization algorithms. In particular, our results suggest  solution accuracy improvements no matter how coarse the gradient compressor is (for arbitrarily large $\epsilon$). To illustrate the main ideas, we consider distributed gradient methods with full gradient communication in this section, and also extend the results for partial gradient communication in Section~\ref{}. 

\iffalse
Even though reducing communication costs, gradient compression cannot reach solution accuracy better than a certain lower bound (see Example \ref{ex:SimpleQ}). Due to the fewer communicated bits, its implementations on optimization algorithms show significant degradation in both accuracy and convergence speed (too coarse compression can even lead to divergence in the extreme cases), \cite{gradientcompression2018,seide20141}. To overcome this communication-accuracy trade-off,  error compensation can recover almost full-accuracy optimums based on low-precision training by gradient compression, \cite{seide20141,strom2015scalable}.
\fi

To overcome significant degradation in both accuracy and convergence speed by
low-precision training with too crude gradient compression, error compensation is  empirically shown to help recover almost full-accuracy optimum, \cite{seide20141,strom2015scalable}. Rather than naively compressing or quantizing the gradient vector $Q(g_k)$, the error compensation scheme is simply to memorize quantization error and add it back to the current gradient before we apply the compressor, \cite{seide20141,strom2015scalable}. In particular,  we send instead $Q(\alpha_k g_k + A_k e_k)$, where 
\begin{align}\label{eqn:ECupdate}
e_{k+1} = \beta_k g_k + A_k e_k - Q(\alpha_k g_k + A_k e_k), 
\end{align}
given $A_k\in\mathbb{R}^{d\times d}$ is positive definite, $\alpha_k,\beta_k > 0$, and $e_0 = \mathbf{0}$. Several works consider special cases of the error compensation update \eqref{eqn:ECupdate} as described below:
%
%
%
\begin{itemize} 
\item The update \eqref{eqn:ECupdate} with $A_k= I$ and $\beta_k =\alpha_k$ is considered in  \cite{Stich2018}.
\item The update \eqref{eqn:ECupdate} with $A_k= I$, $\beta_k = \beta$ and $\alpha_k=\alpha$ is considered in \cite{wu2018error}.
\item The update \eqref{eqn:ECupdate} with $A_k= I$ and $\beta_k =\alpha_k =\beta \in (0,1)$ is considered in \cite{alistarh2018convergence,2019arXiv190109847P}. 
\item The update \eqref{eqn:ECupdate} with $A_k = I -\alpha H_k$, $\beta_k = \alpha_k = 1$, and $H_k$ is the Hessian information associated with the gradient $g_k$ is considered in \cite{ourICASSPworks}.
\end{itemize}
%
%
%
%

% Then, recent works 
Error compensation has been extensively studied on different optimization algorithms; see \emph{e.g.}, in  \cite{wu2018error,Stich2018,alistarh2018convergence}. Many works (\emph{e.g.}, in \cite{wu2018error, alistarh2018convergence}) analyzed the convergence rate results of error-compensated compressed gradient descent algorithms, but did not prove its acceleration over the non-compensated algorithms. Stich \emph{et al.} \cite{Stich2018,2019arXiv190109847P} shows that deterministic error-compensated gradient compression guarantees convergence, while non-compensated compression leads to divergence. However, the analysis is valid for centralized algorithms and is limited for optimization problems under bounded gradient assumptions, and also the deterministic compressors which produce quantization error smaller than magnitude of the full precision vector. Khirirat \emph{et al.} \cite{ourICASSPworks} shows the solution accuracy gained from the error compensation scheme especially for ill-conditioned strongly convex quadratic optimization.


This paper is interested in error compensation \eqref{eqn:ECupdate}  with $A_k = I$ and $\beta_k =\alpha_k= 1$ (as studied \emph{e.g.} in \cite{aji2017sparse,strom2015scalable}), since it is shown to have better empirical convergence performance than other variations in \cite{wu2018error,alistarh2018convergence,Stich2018} (see Section \ref{sec:numericalresults}). In addition, our theoretical results apply for both centralized and distributed algorithms, and explicitly show that error-compensated gradient compression using the $\epsilon-$stochastic compressor with arbitrary precision achieves the better solution accuracy than the non-compensated one. In essence, the error compensation reduces quantization error from $\mathcal{O}(\gamma)$ to $\mathcal{O}(\gamma^2)$ as the iteration counts increase.



\Sindri{I prefer to not include the discussion below on directly compressing the gradient and Theorems 1 and 2 here. 
         We have already discussed direct gradient compression in previous section when we presented lower bound, it is a bit confusing to discuss this here again, especially since we have promised some improvements on this scheme. 
       I suggest moving these results after the lower bound in Example 3.  
       It would be best if we can make these lower bounds tight, so there is a direct comparison between the lower bounds and the theorem.  Also I prefer to have these all as one theorem to keep the message clean.}


\SK{Remove these paragraphs}
To this end, we start by studying compressed gradient descent (CGD) which forms the following iteration
%
%
\begin{align}\label{eqn:CGD}
x_{k+1} = x_k - \gamma Q\left( \nabla f(x_k) \right)
\end{align}
given the fixed positive step-size $\gamma$ and the initial point $x_0\in\mathbb{R}^d$. To facilitate our analysis, we make standard assumptions on families of loss functions. 



\Sindri{I prefer to define these (convex, strongly convex, $L$-smooth) in the beginning of the paper, we can have a section in the introduction called Notation and Definitions or something similar.  We need to keep the message clean, we have promised some results  and need to go to them  quickly and without to many detours. 
 Most readers  have limited patience and will stop reading if we don't  get to the main message quickly. }
\begin{assumption}\label{assum:f_iLipsmooth}
Each loss function $f_i:\mathbb{R}^d\rightarrow\mathbb{R}$ is $L-$smooth if there exists a positive constant $L$ such that 
\begin{align*}
f_i(y) \leq f_i(x) + \langle \nabla f_i(x),y-x \rangle + \frac{L}{2}\| y-x \|^2, \quad \forall x,y\in\mathbb{R}^d.
\end{align*}
\end{assumption}


\begin{assumption}\label{assum:fiConvex}
Each loss function $f_i$ is convex, i.e. 
\begin{align*}
f_i(x) \geq f_i(y) + \langle \nabla f_i(y), x-y \rangle, \quad \forall x,y\in\mathbb{R}^d.
\end{align*}
\end{assumption}

From Assumptions \ref{assum:f_iLipsmooth} and \ref{assum:fiConvex}, it is easy to show that the whole objective function $f$ is also $L-$smooth and convex, respectively. We now state the results:





\begin{theorem}\label{thm:CGD_convex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:f_iLipsmooth} and \ref{assum:fiConvex}. 
\Sindri{ It is not good to say under Assumptions 1 and 2 here. Most readers  know what convex and $L$-smooth means, but have probably forgotten what our Assumptions 1 and 2 are and will now have to go and look for the definition. }
 Assume that the compressor is UBEC and that $\gamma < 1/L$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:CGD} satisfy 
%
%
\begin{align*}
\mathbf{E} \{  f(\bar x_k) - f(x^\star)\} \leq \frac{0.5}{k+1}\cdot\frac{1}{\gamma}\frac{1}{1-L\gamma} \|  x_0 - x^\star\|^2 +\frac{\gamma}{1-L\gamma}\epsilon,
\end{align*}
%
%
where $\bar x_k = (1/(k+1))\sum_{l=0}^k x_l$.
%
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:CGD_convex}.
\end{proof}

\begin{theorem}\label{thm:CGD_nonconvex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:f_iLipsmooth}. Assume that the compressor is UBEC and that $\gamma < 1/L$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:CGD} satisfy 
%
%
\begin{align*}
\min_{l\in\{0,1,\ldots,k\}}\mathbf{E} \| \nabla f(x_l) \|^2 
\leq \frac{1}{k+1}\cdot\frac{1}{\gamma} \frac{1}{1-\gamma L}\left( f(x_0) - f(x^\star)\right) + \frac{2L\gamma}{1- \gamma L} \epsilon.
\end{align*}
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:CGD_nonconvex}.
\end{proof}

From Theorems 1 and 2, we reach the sub-linear convergence rate of CGD, and recover the GD convergence when we let $\epsilon=0$.

\SK{Remove these paragraphs until this line.}


To this end, we consider error-compensated compressed gradient descent (EC-CGD)
%
%
%
\begin{equation}\label{eqn:ECCGD}
\begin{split}
x_{k+1} = x_k - \gamma Q\left(\nabla f(x_k)  + e_k \right), \quad \text{and} \\ 
e_{k+1} = \nabla f(x_k)  + e_k - Q\left(\nabla f(x_k)  + e_k \right)
\end{split}
\end{equation}
given $e_0=\mathbf{0}$. The results are given below:
%

\SK{We have to merge Theorems 4 and 5 into one theorem.}

%
\begin{theorem}\label{thm:ECCGD_convex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:f_iLipsmooth} and \ref{assum:fiConvex}. Assume that the compressor is UBEC and that $\gamma < 1/L$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:ECCGD} satisfy 
%
\begin{align*}
\mathbf{E} \{  f(\bar x_k) - f(x^\star)\} 
&\leq \frac{1}{k+1}\cdot\frac{1}{\gamma} \frac{1}{1-L\gamma}\|  x_0  -x^\star \|^2  + \frac{\gamma}{1-L\gamma} 2L\gamma \cdot\epsilon,
\end{align*}
where $\bar x_k = (1/(k+1))\sum_{l=0}^k x_l$
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:ECCGD_convex}.
\end{proof}

\begin{theorem}\label{thm:ECCGD_nonconvex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:f_iLipsmooth}. Assume that the compressor is UBEC and that $\gamma < 1/L$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:ECCGD} satisfy 
%
%
\begin{align*}
\min_{l\in\{0,1,\ldots,k\}}\mathbf{E} \| \nabla f(x_l) \|^2 
\leq \frac{2}{k+1}\cdot\frac{1}{\gamma} \frac{1}{1-L\gamma}\left( f(x_0) - f(x^\star)\right) + \frac{2L\gamma}{1- L \gamma L} 0.5L\gamma\cdot\epsilon.
\end{align*}
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:ECCGD_nonconvex}.
\end{proof}


Even though EC-CGD converges toward the sub-optimum slower than CGD by a factor of $2$, EC-CGD reduces quantization error from $\mathcal{O}(\gamma)$ to $\mathcal{O}(\gamma^2)$ if $\gamma<0.5/L$ and $\gamma < 1/L$ in Theorems  \ref{thm:ECCGD_convex} and \ref{thm:ECCGD_nonconvex}, respectively.


\SK{Remove Section 3.1, but merge discussions into Section 3.2}
\subsection{Compressed SGD}



\Sindri{Like mentioned before, we need to keep the discussion focussed.  I don't think this the right place to motivate stochastic gradient decent, that discussion should be in Section 2.1.2 were we motivate our study. 
 Reviewers/readers are going to be  annoyed to having to read again and again about what they probably know and has already been discussed before.  We should go quickly to our innovation and our results. }

Due to massive scale of datasets, modern machine learning applications focus on solving Problem \eqref{eqn:Problem} when $m$ is extremely large. \emph{Stochastic gradient descent} (SGD) becomes among the most popular randomized optimization algorithms, since it requires low per-iteration cost but guarantees convergence toward the sub-optimum.  To address communication bottleneck, we consider the compressed stochastic gradient descent (CSGD) algorithm 
%
\begin{align}\label{eqn:CSGD}
x_{k+1} = x_k - \gamma Q\left(  \nabla f_{i_k}(x_k)   \right),
\end{align}
where $i_k$ is the index selected randomly selected from uniform distribution, i.e. $p_{i_k}=1/m$. Here, the stochastic gradient $\nabla f_{i_k}(x_k)$ satisfies the unbiased condition, i.e. 
\begin{align*}
 \mathbb{E}_{i_k} \nabla f_{i_k}(x_k) = \nabla f(x_k).
\end{align*}

\Sindri{Do we have results for the more general stochastic gradient where 
$x_{k+1} = x_k - \gamma Q\left(  \nabla_x f(x_k) +\omega_k   \right)$
 and $\mathbb{E} \omega_k = 0$?
 This setting is actually very fitting for compression for dual decomposition. Also, I am afraid that if we are including functions $f_i(\cdot)$ here then people will start to confuse it with the partial gradient method. }

Now, we state the result:
\begin{theorem}\label{thm:CSGD_convex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:f_iLipsmooth} and \ref{assum:fiConvex}. Assume that the compressor is UBEC and that $\gamma < 2/(3L)$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:CSGD} satisfy 
%
%
\begin{align*}
\mathbf{E} \{  f(\bar x_k) - f(x^\star)\} \leq \frac{1}{k+1}\cdot\frac{1}{\gamma}\cdot\frac{1}{2-3L\gamma} \|  x_0 - x^\star\|^2 +\frac{3\gamma}{2-3L\gamma}  (\epsilon+N),
\end{align*}
%
%
where $\bar x_k = (1/(k+1))\sum_{l=0}^k x_l$ and $N = {\max}_{i} \mathbf{E}\| \nabla f_i(x^\star)\|^2$.
%
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:CSGD_convex}.
\end{proof}

Unlike \cite[Theorem 3.4]{alistarh2017qsgd}, Theorem \ref{thm:CSGD_convex} establishes sub-linear convergence of CSGD toward sub-optimum without bounded gradient assumptions. Also, decreasing the step-size leads to slow convergence but low residual error due to stochastic gradient noises and quantization. If we fix the iteration counts $k$, and let the step-size  $\gamma=\mathcal{O}(1/\sqrt{k+1})$ in Theorem \ref{thm:CSGD_convex}, then CSGD converges toward the optimum with rate $\mathcal{O}(1/\sqrt{k+1})$, like SGD convergence presented by \cite[Theorem 6.3]{bubeck2015convex}.

Beforing proving the sub-linear convergence of CSGD for non-convex optimization, we introduce one additional commonly-used assumption. 
%
\begin{assumption}[\cite{lian2015asynchronous,tang2018decentralization,lian2017can}]\label{assum:fiBoundedVarNC}
There exists a positive constant $\sigma$ such that
\begin{align*}
\mathbf{E}\| \nabla f_{i_k}(x) - \nabla f(x) \|^2 \leq \sigma^2, \quad \forall x\in\mathbb{R}^d.
\end{align*}
\end{assumption}
%
Here is the result:
%
\begin{theorem}\label{thm:CSGD_nonconvex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:f_iLipsmooth} and \ref{assum:fiBoundedVarNC}. Assume that the compressor is UBEC and that $\gamma < 2/(3L)$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:CSGD} satisfy 
%
%
\begin{align*}
\min_{l\in\{0,1,\ldots,k\}}\mathbf{E} \| \nabla f(x_l) \|^2 
\leq \frac{1}{k+1}\cdot\frac{1}{\gamma} \frac{1}{1-3 \gamma L/2}\left( f(x_0) - f(x^\star)\right) + \frac{3L\gamma}{1- 3\gamma L/2} (\epsilon +\sigma^2).
\end{align*}
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:CSGD_nonconvex}.
\end{proof}

To improve the solution accuracy, we next consider the error-compensated compressed stochastic gradient descent (EC-CSGD) which forms the iterates according to 
\begin{equation}\label{eqn:EC-CSGD}
\begin{split}
x_{k+1} &= x_k - \gamma Q\left( \nabla f_{i_k}(x_k) + e_k \right), \quad \text{and} \\ 
e_{k+1} &=  \nabla f_{i_k}(x_k) + e_k  - Q\left( \nabla f_{i_k}(x_k) + e_k \right)
\end{split}
\end{equation}
given $e_0=\mathbf{0}.$ Hence, we state the convergence rate results below: 
%
%
%
%
\begin{theorem}\label{thm:ECCSGD_convex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:f_iLipsmooth} and \ref{assum:fiConvex}. Assume that the compressor is UBEC and that $\gamma < 2/(3L)$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:EC-CSGD} satisfy 
%
\begin{align*}
\mathbf{E} \{  f(\bar x_k) - f(x^\star)\} 
&\leq \frac{1.5}{k+1}\cdot\frac{1}{\gamma} \frac{1}{2-3L\gamma}\|  x_0  -x^\star \|^2  + \frac{3\gamma}{2-3L\gamma}(3L\gamma \epsilon/2 + N),
\end{align*}
where $\bar x_k = (1/(k+1))\sum_{l=0}^k x_l$ and $N = {\max}_{i} \mathbf{E}\| \nabla f_i(x^\star)\|^2$.
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:ECCSGD_convex}.
\end{proof}



\begin{theorem}\label{thm:ECCSGD_nonconvex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:f_iLipsmooth} and \ref{assum:fiBoundedVarNC}. Assume that the compressor is UBEC and that $\gamma < 2/(3L)$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:EC-CSGD} satisfy 
%
%
\begin{align*}
\min_{l\in\{0,1,\ldots,k\}}\mathbf{E} \| \nabla f(x_l) \|^2 
\leq \frac{2}{k+1}\cdot\frac{1}{\gamma} \frac{1}{1-3 \gamma L/2}\left( f(x_0) - f(x^\star)\right) + \frac{3L\gamma}{1- 3\gamma L/2} ( L\gamma\epsilon/3 +\sigma^2).
\end{align*}
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:ECCSGD_nonconvex}.
\end{proof}



Theorems \ref{thm:ECCSGD_convex} and \ref{thm:ECCSGD_nonconvex} show slower sub-linear convergence of EC-CSGD than CSGD by $1.5$ and $2$, as shown in Theorems \ref{thm:CSGD_convex} and \ref{thm:CSGD_nonconvex}, respectively. However, EC-CSGD is shown to significantly improve solution accuracy when the number of iterations increases ($k\rightarrow\infty$). In particular, suppose that the residual error is dominated by quantization (i.e. $\epsilon \gg \max(1,2L/3)N$ and $\epsilon \gg \max(1,L/3)\sigma^2$ for convex and non-convex optimization problems, respectively). Then, the quantization error term from EC-CSGD is penalized by $\mathcal{O}(\gamma^2)$ rather than $\mathcal{O}(\gamma)$ from CSGD.


==> Main_Results/centralized_SK_1.tex <==
\section{Error Compensated Gradient Compression} \label{sec:ECGC}

%\Sindri{We need to include more structure here so people can easily understand the main result.  There are \emph{many} ways to do this. Below I am suggesting one way that I think will do the job. We can also discuss other approaches if you like.  }



%\Sindri{We can split the section into the following three subsections. I have written the subsections titles so that people can easily see where to look for different information. For example, if a person wants to get the main idea of our algorithm they go to the first subsection. It is also important that the reader can get the big picture of what he/she is reading. When we read then the brain has  allot of priors on what it is reading.  Therefore, it becomes much easier to read if we make know roughly what to expect.}  

In this section we illustrate how error compensation can improve the direction compression discussed in the previous section.  We illustrate the error compensated gradient methods in subsection~\ref{subsec:ECGC-AI}.  We then provide our main results for  full and partial gradient communication, respectively, in subsections~\ref{subsec:ECGC-FG} and~\ref{subsec:ECGC-PG}.

\subsection{Error Compensation: Algorithm and Illustrative Example}  \label{subsec:ECGC-AI}





%\Sindri{Can you move the relevant information here. We can illustrate the algorithm  and the intuition.  Then we give an illustrate example, which is the quadradic case. }

%\Sindri{For the quadratic case don't just say here are the results for a quadratic problem.  We should illustrate the nice intuition  that can be obtained for the quadraic problem. The algorithm in Equation~\eqref{eqn:ECCGD} will look random to most people. By illustrating how the recursions work on the quadradic problem we show people that we are not doing something random. We are doing something that makes allot of sense by considering a quadiradic problem. Then in later subsections we show that this intuition also works for more general problems.  }


To overcome degradation in convergence performance by naive, direct gradient compression, error compensation can 
recover almost full-accuracy optimal solution~\cite{seide20141,strom2015scalable}. In particular, instead of directly compressing gradient error compensation accounts for memory of quantization errors.


To illustrate the main idea of the error compensation scheme,  we consider the error-compensated compressed gradient descent (EC-CSGD) which follows the iterations according to 
\begin{equation}\label{eqn:ECCSGD}
\begin{aligned}
	x^{k+1} & =x^k - \gamma Q( \nabla g(x^k;\xi^k) + A^k e^k) \\
	e^{k+1} &=  \nabla g(x^k;\xi^k) + A^k e^k - Q( \nabla g(x^k;\xi^k) + A^k e^k),
\end{aligned}
\end{equation}
where $\nabla g(x;\xi)$ is the stochastic gradient. Notice that we recover the variants of error compensation proposed by \cite{alistarh2018convergence,Stich2018} and by \cite{ourICASSPworks} if we let  $A^k=I$ and $A^k=I-\gamma H^k$ where $H^k$ is the Hessian information associated with the stochastic gradient, respectively.


To show why error compensation outperforms direct gradient compression, we again consider the case when $\nabla g(x^k;\xi^k)=\nabla f(x^k)$ and $e^0=0$, and the minimization problem over the quadratic objective function~\eqref{eq:quadOBJ}. In this case, EC-CSGD with $A^k=A_\gamma=I-\gamma H$ is similar to direct gradient compression in Equation~\eqref{eqn:CGD} except we have included the correction term $e^k$ in the gradient update. 
To see the benefits of the correction term we define
$$c^k  =  \nabla f(x^k) - Q(\nabla f(x^k) + A e^k).$$
The error correction step can be re-written as
\begin{align*}
e^{k+1} = c^k + Ae^k, %\quad \replaced{}{\text{or equivalently}  \quad e^k = \sum_{i=0}^{k-1} A^{k-1-i} c^i.}
\end{align*}
which reduces to 
\begin{align*}
  \quad e^k = \sum_{j=0}^{k-1} A^{k-1-j} c^j.
\end{align*}
We can also write the algorithm step equivalently, similarly as in Equation~\eqref{eq:xupdate}, as 
 \begin{align*}
      x^{k+1}=A_{\gamma}x^k-\gamma b+ \gamma c^k
 \end{align*}
 which reduces to 
%By the error correction step, EC-CGD satisfies
%
\begin{align*}
x^{k+1} - x^\star  = A^{k+1} (x^0 - x^\star) +  \gamma \sum_{i=0}^{k} A^{k-i} c^i  = A^{k+1} (x^0 - x^\star) +  \gamma e^{k+1}.
\end{align*}
By error compensation the residual error depends only on the latest quantization error, instead of the accumulation of previous quantization errors.
This in turns helps recover high solution accuracy given proper step-size tuning.  We illustrate this in the following theorem. 



\begin{theorem}\label{thm:ErrorCompensatedSC}
Consider the quadratic optimization problem \eqref{eqn:Problem} with $f(x)=(1/2)x^THx + b^Tx$ where $\mu\cdot I \preceq H \preceq L\cdot I$  for some positive real numbers $\mu,L$.  Assume that $A^k=I-\gamma H$ and $e^0={0}$. Then, the iterates $\{x^k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:ECCGD} with $\omega^k=0$ satisfy
\begin{align*}
    \| x^k - x^\star  \|  \leq \rho^k\| x^0 - x^\star \| + \gamma \epsilon, 
\end{align*}
where 
\begin{align*}
\rho &= \left\{ \begin{array}{ll} 1-1/\kappa & \text{if } \quad \gamma = 1/L \\   1-{2}/{(\kappa+1)} & \text{if }\quad \gamma = 2/(\mu+L)   \end{array}\right.  ,
\end{align*}
and $\kappa = L/\mu$.
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:ErrorCompensatedSC}.
\end{proof}
%
Theorem \ref{thm:ErrorCompensatedSC} implies that error compensation in Equation \eqref{eqn:ECCSGD} achieves the same linear convergence rate as but lower residual error than direct gradient compression as shown in Theorem \ref{thm:CGDQuadratic}, especially for ill-conditioned quadratic optimization problems, \cite{ourICASSPworks}. In particular, error compensation in Equation \eqref{eqn:ECCSGD} with $\gamma=1/L$ and $\gamma=2/(\mu+L)$ reduces quantization error $\kappa$ and $(\kappa+1)/2$, respectively.


Even though limited to quadratic optimization, we next analyze error-compensated stochastic gradient methods under partial gradient communication architectures in the subsequent section. 

\iffalse
\subsection{Full Gradient Communication}   \label{subsec:ECGC-FG}

%\Sindri{Move the relevant text here.  More discussion of the results are needed. What are the implications of the theorem. }

For full gradient communication architecture, we consider the error-compensated compressed stochastic gradient descent (EC-CSGD) which has the following iteration: given  the fixed,positive step-size $\gamma$,  the positive definite matrix $A^k\in\mathbb{R}^{d\times d}$, the initial point $x^0\in\mathbb{R}^d$, and $e^0={0}$,
\begin{equation}\label{eqn:ECCGD}
\begin{split}
x^{k+1} &= x^k - \gamma Q( \nabla g(x^k;\xi^k) + \omega^k + A^k e^k), \quad \text{and}\\
e^{k+1} &=  \nabla g(x^k;\xi^k) + \omega^k + A^k e^k - Q(\nabla g(x^k;\xi^k) + \omega^k + A^k e^k),
\end{split}
\end{equation}
where the stochastic noise satisfies $\mathbf{E}\omega^k=0$ and $\mathbf{E}\| \omega^k \|^2\leq \sigma^2_\omega$, and the stochastic gradient  $\nabla g(x^k;\xi^k)$ satisfies the unbiased property and bounded variance assumption \eqref{eqn:UnbiasedAndBoundedVariance}. Note that EC-CSGD with $A^k=I$ is similar to several works, \emph{e.g.} \cite{2019arXiv190109847P,Stich2018}. 

Motivated by \cite{ourICASSPworks}, we rather study  EC-CSGD with $A^k=I-\gamma H^k$ where $H^k$ is the Hessian matrix associated with the stochastic gradient $\nabla g(x^k;\xi^k)$. Later, our simulation results indicate that our variant outperforms others when the binary compression is used.  Next, we state the results of EC-CSGD convergence. 

\begin{theorem}\label{thm:ECCGD}
Consider an optimization problem \eqref{eqn:Problem} and the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:ECCGD} with $A^k = I -\gamma H^k$. Assume that the compressor is $\epsilon-$deterministic, and that $H^k \preceq \Lambda I$ for a positive constant $\Lambda$. If the whole objective function $f$ is $L-$smooth and $\gamma< \min\left\{ 1/\Lambda , 1/(4L)\right\}$, then 
\begin{align*}
\mathop{\min}\limits_{l\in[0,k]} \mathbf{E} \| \nabla f(x^l) \|^2 
& \leq \frac{1}{k+1}\frac{2}{\gamma}\frac{1}{1-4L\gamma}\left( f( x^{0}) - f(x^\star) \right) \\ 
& \hspace{0.4cm} + \frac{ {L^2} +  {\Lambda^2} + 4L\Lambda^2 \gamma}{1-4L\gamma}\gamma^2\epsilon^2 + \frac{4L}{1-4L\gamma} \gamma(\sigma_v^2 + \sigma_\omega^2).
\end{align*}
%
If  $f$ is also $\mu-$strongly convex and $\gamma< \min\left\{ 1/\Lambda, (1-\beta)/(4L) \right\}$ where $0<\beta<1$, then 
\begin{align*}
\mathbf{E}\left(f(\bar x^k) - f(x^\star) \right)
 & \leq \frac{1}{k+1}\frac{1}{2\gamma}\frac{1}{1-\beta-4L\gamma}\|  x^{0} - x^\star \|^2  \\
&\hspace{0.4cm} + \frac{\mu + L/\beta + (2/\mu+4\gamma)\Lambda^2 }{2(1-\beta-4L\gamma)}\gamma^2 \epsilon^2+ \frac{2}{1-\beta-4L\gamma}\gamma(\sigma^2_v + \sigma_\omega^2 ) ,
\end{align*}
where $\bar x^k = \sum_{l=0}^k x^l/(k+1).$
\end{theorem}
\begin{proof}
See Appendix \ref{app:ECCGD}.
\end{proof}

Unlike \cite{Stich2018,2019arXiv190109847P}, Theorem \ref{thm:ECCGD} establishes the convergence of EC-CSGD using the compression operator without any contraction property and without the bounded gradient assumption  for strongly convex and non-convex optimization. Even though the solution accuracy depends on stochastic gradient, the stochastic noise and the precision of compression operators, we show that error compensation reduces the quantization error by $\mathcal{O}(\gamma^2)$. To validate this point, consider the case when $k\rightarrow\infty$, and $\nabla g(x;\xi) = \nabla f(x)$ and $\omega=0$ ($\sigma_v^2=\sigma_\omega^2=0$). Then, the upper bound of $\| \nabla f(x^k) \|^2$ and $f(\bar x^k) - f(x^\star)$ are $(L^2+\Lambda^2+4L\Lambda^2\gamma)/(1-4L\gamma)\cdot \gamma^2\epsilon^2$ and $0.5(\mu+L/\beta+(2/\mu+4\gamma)\Lambda^2)/(1-\beta-4L\gamma)\cdot \gamma^2\epsilon^2$. Therefore, error compensation recovers arbitrarily highly accurate solution, especially when the step-size is small. 

Furthermore, we easily establish the convergence of EC-CGD \eqref{eqn:ECCGD_quad}, when we let  $H^k = H$, and  $\nabla g(x;\xi) = \nabla f(x)$ and $\omega=0$ ($\sigma_v^2=\sigma_\omega^2=0$) in Theorem \ref{thm:ECCGD}. The convergence of EC-CSGD using error compensation schemes by \cite{alistarh2018convergence,Stich2018} and by \cite{ourICASSPworks} can also be established, when we let $H^k= \mathbf{0}$ and $H^k = \nabla^2 f(x^k)$ in Theorem \ref{thm:ECCGD}, respectively. Note that $ \mu I \preceq \nabla^2 f(x) \preceq L I$ for $x\in\mathbb{R}^d$ if the twice-continuously differentiable objective function $f$ is  $\mu$-strongly convex and $L-$smooth, \cite{friedlander2012hybrid}. 
\fi


%
%
%
%
%

\iffalse
\Sindri{This paragraph below on comparing to other work breaks  the flow of the section.  We can put it in the end of subsection~\ref{subsec:ECGC-AI} as a remark.}
Several works have \replaced{}{extensively} analyzed convergence rates of error compensated gradient descent methods for full gradient and partial gradient communication architectures; see \emph{e.g.}, in \cite{Stich2018,2019arXiv190109847P,ourICASSPworks} and \cite{wu2018error,alistarh2018convergence}, respectively. In addition, many works consider special cases of EC-CGD \eqref{eqn:ECCGD} such as   EC-CGD with $A^k= I$, $\gamma=1$ and EC-CGD with $A^k = I -\gamma H^k$, $\alpha = 1$, and $H^k$ is the Hessian information associated with the gradient $\nabla f(x^k)$ by \cite{alistarh2018convergence,2019arXiv190109847P} and by \cite{ourICASSPworks}, respectively. 
\fi
%
%
\iffalse
% Then, recent works 
Error compensation has been extensively studied on gradient-based optimization algorithms under centralized and distributed architectures; see \emph{e.g.}, in \cite{Stich2018,2019arXiv190109847P,ourICASSPworks} and \cite{wu2018error,alistarh2018convergence}, respectively.  Stich \emph{et al.} \cite{Stich2018,2019arXiv190109847P} proves error-compensated compressed SGD while shows the divergence of naive deterministic gradient compression by simple counter-examples, while Khirirat \emph{et al.} \cite{ourICASSPworks} proves that error compensation on centralized gradient algorithms improves solution accuracy by the condition number of the problem for quadratic optimization problems. In the parameter server framework,  error compensation is proven to help compressed algorithms achieve almost the same convergence rate as their full-precision counterparts,  \emph{e.g.}, in \cite{wu2018error,alistarh2018convergence}.
\fi
\iffalse
In this paper, we study one variant of error compensation schemes by  \cite{ourICASSPworks}. In particular, our results indicate the reduce in quantization error  by $\mathcal{O}(\gamma^2)$ as the iteration counts increase. Later, our empirical results are shown to validate this indication and also to outperform other error compensation schemes  by \cite{alistarh2018convergence,2019arXiv190109847P}  in Section \ref{sec:numericalresults}.
\fi
\iffalse
convergence of GD and distributed SGD using the error compensation scheme by  \cite{ourICASSPworks}, without the assumptions of bounded gradient and   the mergeability property of the deterministic compressor (see \cite[Assumption 1]{alistarh2018convergence}). 

In essence, we explicitly show that error compensation on the $\epsilon-$deterministic compressor reduces the residual error by $\mathcal{O}(\gamma^2)$ as the iteration counts increase. The empirical results indicate that compensation scheme proposed by \cite{ourICASSPworks} recovers significantly high solution accuracy  than the counterparts proposed by \cite{alistarh2018convergence,2019arXiv190109847P}, as shown in Section \ref{sec:numericalresults}.
\fi












%======================== old ===============================%
\iffalse
\subsection{Compressed SGD}



\Sindri{Like mentioned before, we need to keep the discussion focussed.  I don't think this the right place to motivate stochastic gradient decent, that discussion should be in Section 2.1.2 were we motivate our study. 
 Reviewers/readers are going to be  annoyed to having to read again and again about what they probably know and has already been discussed before.  We should go quickly to our innovation and our results. }

Due to massive scale of datasets, modern machine learning applications focus on solving Problem \eqref{eqn:Problem} when $m$ is extremely large. \emph{Stochastic gradient descent} (SGD) becomes among the most popular randomized optimization algorithms, since it requires low per-iteration cost but guarantees convergence toward the sub-optimum.  To address communication bottleneck, we consider the compressed stochastic gradient descent (CSGD) algorithm 
%
\begin{align}\label{eqn:CSGD}
x_{k+1} = x_k - \gamma Q\left(  \nabla f_{i_k}(x_k)   \right),
\end{align}
where $i_k$ is the index selected randomly selected from uniform distribution, i.e. $p_{i_k}=1/m$. Here, the stochastic gradient $\nabla f_{i_k}(x_k)$ satisfies the unbiased condition, i.e. 
\begin{align*}
 \mathbb{E}_{i_k} \nabla f_{i_k}(x_k) = \nabla f(x_k).
\end{align*}

\Sindri{Do we have results for the more general stochastic gradient where 
$x_{k+1} = x_k - \gamma Q\left(  \nabla_x f(x_k) +\omega_k   \right)$
 and $\mathbb{E} \omega_k = 0$?
 This setting is actually very fitting for compression for dual decomposition. Also, I am afraid that if we are including functions $f_i(\cdot)$ here then people will start to confuse it with the partial gradient method. }

Now, we state the result:
\begin{theorem}\label{thm:CSGD_convex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:f_iLipsmooth} and \ref{assum:fiConvex}. Assume that the compressor is UBEC and that $\gamma < 2/(3L)$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:CSGD} satisfy 
%
%
\begin{align*}
\mathbf{E} \{  f(\bar x_k) - f(x^\star)\} \leq \frac{1}{k+1}\cdot\frac{1}{\gamma}\cdot\frac{1}{2-3L\gamma} \|  x_0 - x^\star\|^2 +\frac{3\gamma}{2-3L\gamma}  (\epsilon+N),
\end{align*}
%
%
where $\bar x_k = (1/(k+1))\sum_{l=0}^k x_l$ and $N = {\max}_{i} \mathbf{E}\| \nabla f_i(x^\star)\|^2$.
%
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:CSGD_convex}.
\end{proof}

Unlike \cite[Theorem 3.4]{alistarh2017qsgd}, Theorem \ref{thm:CSGD_convex} establishes sub-linear convergence of CSGD toward sub-optimum without bounded gradient assumptions. Also, decreasing the step-size leads to slow convergence but low residual error due to stochastic gradient noises and quantization. If we fix the iteration counts $k$, and let the step-size  $\gamma=\mathcal{O}(1/\sqrt{k+1})$ in Theorem \ref{thm:CSGD_convex}, then CSGD converges toward the optimum with rate $\mathcal{O}(1/\sqrt{k+1})$, like SGD convergence presented by \cite[Theorem 6.3]{bubeck2015convex}.

Beforing proving the sub-linear convergence of CSGD for non-convex optimization, we introduce one additional commonly-used assumption. 
%
\begin{assumption}[\cite{lian2015asynchronous,tang2018decentralization,lian2017can}]\label{assum:fiBoundedVarNC}
There exists a positive constant $\sigma$ such that
\begin{align*}
\mathbf{E}\| \nabla f_{i_k}(x) - \nabla f(x) \|^2 \leq \sigma^2, \quad \forall x\in\mathbb{R}^d.
\end{align*}
\end{assumption}
%
Here is the result:
%
\begin{theorem}\label{thm:CSGD_nonconvex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:f_iLipsmooth} and \ref{assum:fiBoundedVarNC}. Assume that the compressor is UBEC and that $\gamma < 2/(3L)$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:CSGD} satisfy 
%
%
\begin{align*}
\min_{l\in\{0,1,\ldots,k\}}\mathbf{E} \| \nabla f(x_l) \|^2 
\leq \frac{1}{k+1}\cdot\frac{1}{\gamma} \frac{1}{1-3 \gamma L/2}\left( f(x_0) - f(x^\star)\right) + \frac{3L\gamma}{1- 3\gamma L/2} (\epsilon +\sigma^2).
\end{align*}
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:CSGD_nonconvex}.
\end{proof}

To improve the solution accuracy, we next consider the error-compensated compressed stochastic gradient descent (EC-CSGD) which forms the iterates according to 
\begin{equation}\label{eqn:EC-CSGD}
\begin{split}
x_{k+1} &= x_k - \gamma Q\left( \nabla f_{i_k}(x_k) + e_k \right), \quad \text{and} \\ 
e_{k+1} &=  \nabla f_{i_k}(x_k) + e_k  - Q\left( \nabla f_{i_k}(x_k) + e_k \right)
\end{split}
\end{equation}
given $e_0=\mathbf{0}.$ Hence, we state the convergence rate results below: 
%
%
%
%
\begin{theorem}\label{thm:ECCSGD_convex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:f_iLipsmooth} and \ref{assum:fiConvex}. Assume that the compressor is UBEC and that $\gamma < 2/(3L)$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:EC-CSGD} satisfy 
%
\begin{align*}
\mathbf{E} \{  f(\bar x_k) - f(x^\star)\} 
&\leq \frac{1.5}{k+1}\cdot\frac{1}{\gamma} \frac{1}{2-3L\gamma}\|  x_0  -x^\star \|^2  + \frac{3\gamma}{2-3L\gamma}(3L\gamma \epsilon/2 + N),
\end{align*}
where $\bar x_k = (1/(k+1))\sum_{l=0}^k x_l$ and $N = {\max}_{i} \mathbf{E}\| \nabla f_i(x^\star)\|^2$.
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:ECCSGD_convex}.
\end{proof}



\begin{theorem}\label{thm:ECCSGD_nonconvex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:f_iLipsmooth} and \ref{assum:fiBoundedVarNC}. Assume that the compressor is UBEC and that $\gamma < 2/(3L)$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:EC-CSGD} satisfy 
%
%
\begin{align*}
\min_{l\in\{0,1,\ldots,k\}}\mathbf{E} \| \nabla f(x_l) \|^2 
\leq \frac{2}{k+1}\cdot\frac{1}{\gamma} \frac{1}{1-3 \gamma L/2}\left( f(x_0) - f(x^\star)\right) + \frac{3L\gamma}{1- 3\gamma L/2} ( L\gamma\epsilon/3 +\sigma^2).
\end{align*}
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:ECCSGD_nonconvex}.
\end{proof}



Theorems \ref{thm:ECCSGD_convex} and \ref{thm:ECCSGD_nonconvex} show slower sub-linear convergence of EC-CSGD than CSGD by $1.5$ and $2$, as shown in Theorems \ref{thm:CSGD_convex} and \ref{thm:CSGD_nonconvex}, respectively. However, EC-CSGD is shown to significantly improve solution accuracy when the number of iterations increases ($k\rightarrow\infty$). In particular, suppose that the residual error is dominated by quantization (i.e. $\epsilon \gg \max(1,2L/3)N$ and $\epsilon \gg \max(1,L/3)\sigma^2$ for convex and non-convex optimization problems, respectively). Then, the quantization error term from EC-CSGD is penalized by $\mathcal{O}(\gamma^2)$ rather than $\mathcal{O}(\gamma)$ from CSGD.
\fi
%======================== old ===============================%

==> Main_Results/distributed.tex <==
%=========================================================%
%  Section: distributed GD
%=========================================================%
\subsection{Distributed Compressed SGD \SK{Extension to Partial Gradient Compression}}\label{sec:DCSGD}
%
%
%
\SK{We should start with: In this section, we show that error compensation can be applied to distributed gradient methods with partial gradient communication to significantly improve solution accuracy.}
%
%
We start by considering the distributed compressed stochastic gradient descent algorithm (D-CSGD)
\begin{align}\label{eqn:QDGD}
x_{k+1} = x_k - \gamma \frac{1}{m}\sum_{i=1}^m Q(\nabla g_i(x_k;\xi_i)). 
\end{align}
Here, the compressed stochastic gradient $Q(\nabla g_i(x_k;\xi_i))$ preserves the unbiased property, i.e. 
\begin{align*}
\mathbf{E} \{ Q(\nabla g_i(x;\xi_i)) \} = \nabla f_i(x).
\end{align*}

Before providing the analysis, we introduce typical assumptions on $g_i(x;\xi_i)$. 
\begin{assumption}[\cite{nguyen2018sgd}]\label{assum:LonGi}
Each $g_i(x;\xi_i)$ is $L-$smooth for every realization of $\xi_i$, i.e. 
\begin{align}
\| \nabla g_i(x;\xi_i) -\nabla g_i(y;\xi_i) \| \leq L \| x-y\|, \quad \forall x,y\in\mathbb{R}^d.
\end{align}
\end{assumption}

Note that Assumption \ref{assum:LonGi} implies that $f_i$ and $f$ are smooth with $L$, \cite{nguyen2018sgd,khirirat2018distributed}. 

\begin{assumption}[\cite{nguyen2018sgd}]\label{assum:GiConvex}
Each $g_i(x;\xi_i)$ is convex for every realization of $\xi_i$, i.e. 
\begin{align}
g_i(x;\xi_i) \geq g_i(y;\xi_i) + \langle \nabla g_i(y;\xi_i), x-y \rangle, \quad \forall x,y\in\mathbb{R}^d.
\end{align}
\end{assumption}



\begin{assumption}[\cite{lian2017can,pu2018distributed}]\label{assum:GiBoundedVariance}
Each $\nabla g_i(x;\xi_i)$ has bounded variance, i.e. 
\begin{align}
\mathbf{E}\| \nabla g_i(x;\xi_i)  - \nabla f_i(x) \|^2 \leq \sigma^2, \quad \forall x\in\mathbb{R}^d.
\end{align}
\end{assumption}

Unlike \cite[Assumption 1]{lian2015asynchronous} and
\cite[Assumption 3]{feyzmahdavian2016asynchronous}, Assumption \ref{assum:GiBoundedVariance} simply assumes similarity between the local gradient and its stochastic oracle, which allows for complete difference between the whole data and local data  distributions.



Now, we provide the results: 

\begin{theorem}\label{thm:distCSGD_convex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:LonGi} and \ref{assum:GiConvex}. Assume that the compressor is UBEC and that $\gamma < 2/(3L)$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:QDGD} satisfy 
%
%
\begin{align*}
\mathbf{E} \{  f(\bar x_k) - f(x^\star)\} \leq \frac{1}{k+1}\cdot\frac{1}{\gamma}\cdot\frac{1}{2-3L\gamma} \|  x_0 - x^\star\|^2 +\frac{3\gamma}{2-3L\gamma}  (\epsilon+N),
\end{align*}
%
%
where $\bar x_k = (1/(k+1))\sum_{l=0}^k x_l$ and $N = \mathbf{E}\| (1/m)\sum_{i=1}^m\nabla g_i(x^\star;\xi_i)\|^2$.
%
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:distCSGD_convex}.
\end{proof}



\SK{sub-linear convergence rate toward sub-optimum without bounded gradient assumptions.}

\SK{decreasing the step-size leads to slow convergence but low residual error.}


\SK{We add discussions when $m=1$ from C-SGD.}

\SK{Consider the mini-batch SGD with $m=1$, which is the centralized mini-batch SGD (running on one computer node). If we further fix the iteration count $k$, and set the step-size $\gamma=\mathcal{O}(1/\sqrt{k+1})$, then Theorem implies the convergence of centralized mini-batch SGD with rate $\mathcal{O}(1/\sqrt{k+1})$ comparable to \cite{}. }


\SK{We can also extend the result for the non-convex optimization as shown below:}

\begin{theorem}\label{thm:distCSGD_nonconvex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:LonGi} and \ref{assum:GiBoundedVariance}. Assume that the compressor is UBEC and that $\gamma < 2/(3L)$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:QDGD} satisfy 
%
%
\begin{align*}
\min_{l\in\{0,1,\ldots,k\}}\mathbf{E} \| \nabla f(x_l) \|^2 
\leq \frac{1}{k+1}\cdot\frac{1}{\gamma} \frac{1}{1-3 \gamma L/2}\left( f(x_0) - f(x^\star)\right) + \frac{3L\gamma}{1- 3\gamma L/2} (\epsilon +\sigma^2).
\end{align*}
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:distCSGD_nonconvex}.
\end{proof}

Theorems \ref{thm:distCSGD_convex} and \ref{thm:distCSGD_nonconvex} establish the convergence of D-CSGD where each work accesses to its local function $f_i$ which can be
completely different from one another, unlike \cite[Theorem D.1]{alistarh2017qsgd} and \cite{lian2015asynchronous}. 




In addition, if all worker nodes compute the gradient based on its whole local data (i.e. $\nabla g_i(x;\xi_i) = \nabla f_i(x)$), then the residual error results only from quantization (since $N=0$ and $\sigma^2=0$ from Theorems \ref{thm:distCSGD_convex} and \ref{thm:distCSGD_nonconvex}). 







To show its better performance, we consider the distributed error-compensated compressed stochastic gradient descent (D-EC-CSGD)
\begin{equation}\label{eqn:DECCSGD}
\begin{split}
x_{k+1} &= x_k - \gamma\frac{1}{m}\sum_{i=1}^m Q(\nabla g_i(x_k;\xi_i) + e_k^i), \quad \text{and}\\
e_{k+1}^i & = \nabla g_i(x_k;\xi_i) + e_k^i - Q(\nabla g_i(x_k;\xi_i) + e_k^i), \quad \text{for} \quad i=1,2,\ldots,m.
\end{split}
\end{equation} 
%
%
Now, we state the results:
%
%
%
\begin{theorem}\label{thm:distEC-CSGD_convex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:LonGi} and \ref{assum:GiConvex}. Assume that the compressor is UBEC and that $\gamma < 2/(3L)$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:DECCSGD} satisfy 
%
\begin{align*}
\mathbf{E} \{  f(\bar x_k) - f(x^\star)\} 
&\leq \frac{1.5}{k+1}\cdot\frac{1}{\gamma} \frac{1}{2-3L\gamma}\|  x_0  -x^\star \|^2  + \frac{3\gamma}{2-3L\gamma}(3L\gamma \epsilon/2 + N),
\end{align*}
where $\bar x_k = (1/(k+1))\sum_{l=0}^k x_l$ and $N = \mathbf{E} \left\| (1/m) \sum_{i=1}^m g_i(x^\star;\xi_i) \right\|^2.$
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:distEC-CSGD_convex}.
\end{proof}


\begin{theorem}\label{thm:distEC-CSGD_nonconvex}
Consider an optimization problem \eqref{eqn:Problem} under Assumptions \ref{assum:LonGi} and \ref{assum:GiBoundedVariance}. Assume that the compressor is UBEC and that $\gamma < 2/(3L)$. Then, the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by  \eqref{eqn:DECCSGD} satisfy 
%
%
\begin{align*}
\min_{l\in\{0,1,\ldots,k\}}\mathbf{E} \| \nabla f(x_l) \|^2 
\leq \frac{2}{k+1}\cdot\frac{1}{\gamma} \frac{1}{1-3 \gamma L/2}\left( f(x_0) - f(x^\star)\right) + \frac{3L\gamma}{1- 3\gamma L/2} ( L\gamma\epsilon/3 +\sigma^2).
\end{align*}
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:distEC-CSGD_nonconvex}.
\end{proof}

While D-EC-CSGD has been analyzed for strongly convex quadratic optimization in \cite{wu2018error}, Theorems \ref{thm:distEC-CSGD_convex} and \ref{thm:distEC-CSGD_nonconvex} establish the D-EC-CSGD convergence for (non-)convex optimization over more general classes of loss functions. 

\SK{There are two cases which error compensation improves solution accuracy. 
\begin{itemize}
\item dominance of quantization over stochastic noise, or 
\item all worker nodes compute the gradient based on its whole local data (i.e. $\nabla g_i(x;\xi_i) = \nabla f_i(x)$).
\end{itemize}
}

\iffalse
If all worker nodes compute the gradient based on its whole local data (i.e. $\nabla g_i(x;\xi_i) = \nabla f_i(x)$), then the quantization error reduces from $\mathcal{O}(\gamma)$ to $\mathcal{O}(\gamma^2)$.
\fi









==> Main_Results/distributed_SK_1.tex <==
%=========================================================%
%  Section: distributed GD
%=========================================================%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Texts begin here 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Partial Gradient Communication}   \label{subsec:ECGC-PG}

%\Sindri{Move the relevant text here.  More discussion of the results are needed.}

In this section, we study the benefit of error compensation for partial gradient communication architecture by considering  the distributed error-compensated compressed stochastic gradient descent (D-EC-CSGD) which performs the following update:
\begin{equation}\label{eqn:DECCSGD}
\begin{split}
x^{k+1} &= x^k - \gamma\frac{1}{n}\sum_{i=1}^n Q(\nabla g_i(x^k;\xi_i^k) + A_i^k e_i^k), \quad \text{and}\\
e_{i}^{k+1} & = \nabla g_i(x^k;\xi_i^k) + A_i^k e_i^k - Q(\nabla g_i(x^k;\xi_i^k) + A_i^k e_i^k), \quad \text{for} \quad i=1,2,\ldots,n.
\end{split}
\end{equation} 
Here, each $\nabla g_i(x;\xi_i)$ again satisfies the unbiased property and the bounded variance assumption. As similarly shown in Theorem  \ref{thm:ErrorCompensatedSC},  the following theorem shows why error compensation outperforms direct gradient compression.



%Note that D-EC-CSGD with $A_i^k=I$ is similar to \cite{wu2018error}, and EC-CSGD is the special case of D-EC-CSGD with $n=1$. Next, we provide D-EC-CSGD convergence as shown below: 
%
%
\begin{theorem}\label{thm:distEC-CSGD_convex}
Consider an optimization problem \eqref{eqn:Problem} and the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:DECCSGD} with $A^k_i = I -\gamma H^k_i$. Assume that the compressor is $\epsilon-$deterministic, and that $H^k_i \preceq \Lambda I$ for a positive constant $\Lambda$. If the whole objective function $f$ is $L-$smooth and $\gamma< \min\left\{ 1/\Lambda , 1/(4L)\right\}$, then 
\begin{align*}
\mathop{\min}\limits_{l\in[0,k]} \mathbf{E} \| \nabla f(x^l) \|^2 
& \leq \frac{1}{k+1}\frac{2}{\gamma}\frac{1}{1-4L\gamma}\left( f( x^{0}) - f(x^\star) \right) \\ 
& \hspace{0.4cm} + \frac{ {L^2} +  {\Lambda^2} + 4L\Lambda^2 \gamma}{1-4L\gamma}\gamma^2\epsilon^2 + \frac{4L}{1-4L\gamma} \gamma(\sigma_v^2 + \sigma_\omega^2).
\end{align*}
%
If  $f$ is also $\mu-$strongly convex and $\gamma< \min\left\{ 1/\Lambda, (1-\beta)/(4L) \right\}$ where $0<\beta<1$, then 
\begin{align*}
\mathbf{E}\left(f(\bar x^k) - f(x^\star) \right)
 & \leq \frac{1}{k+1}\frac{1}{2\gamma}\frac{1}{1-\beta-4L\gamma}\|  x^{0} - x^\star \|^2  \\
&\hspace{0.4cm} + \frac{\mu + L/\beta + (2/\mu+4\gamma)\Lambda^2 }{2(1-\beta-4L\gamma)}\gamma^2 \epsilon^2+ \frac{2}{1-\beta-4L\gamma}\gamma(\sigma^2_v + \sigma_\omega^2 ) ,
\end{align*}
where $\bar x^k = \sum_{l=0}^k x^l/(k+1).$
\end{theorem}
\begin{proof}
See Appendix \ref{app:thm:distEC-CSGD}.
\end{proof}
\iffalse
Consider the case when $k\rightarrow\infty$ and $\nabla g_i(x;\xi_i)=\nabla f_i(x)$ (i.e. $\sigma^2=0$ and $N=0$).  D-EC-CSGD reduces quantization error by $\mathcal{O}(\gamma^2)$, unlike D-CSGD. In addition, 
\fi
%
%
%
%
%
% 
This theorem shows that error compensation in D-EC-CSGD can recover arbitrarily high solution accuracy  unlike direct compression shown in Theorem \ref{thm:distCSGD_convex}. In particular, error compensation, unlike direct compression, has quantization error which can be bounded by $\mathcal{O}(\gamma^2)\epsilon^2$. Therefore, the residual error related to both stochastic gradient noise $\sigma$ and precision of quantization $\epsilon$ can diminish toward zero with diminishing step-size from Theorem \ref{thm:distEC-CSGD_convex}. 

When we let  $H_i^k = \mathbf{0}$  in Theorem \ref{thm:distEC-CSGD_convex}, we can also recover the convergence results of D-EC-CSGD using error compensation variants proposed by \cite{alistarh2018convergence,wu2018error} without the mergeability assumption and without the unbiasedness of the compression operators (see \emph{e.g.}, in \cite[Assumption 1]{alistarh2018convergence} and \cite[Lemma 1]{wu2018error}, respectively). Furthermore, we establish convergence results of D-EC-CSGD using error compensation proposed by~\cite{ourICASSPworks} when we let $H_i^k$ be associated Hessian information of the stochastic gradient $\nabla g_i(x^k;\xi_i^k)$.


%However, we show that the error compensation scheme motivated by \cite{ourICASSPworks} ($H_i^k$ is the Hessian information associated with the stochastic gradient $\nabla g_i(x^k;\xi^k_i)$) outperforms others when the binary compression is used in the next section.







==> Main_Results/distributed_SK_2__Sindri_Magn__sson_s_conflicted_copy_2019-09-16_.tex <==
%=========================================================%
%  Section: distributed GD
%=========================================================%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Texts begin here 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Partial Gradient Communication}   \label{subsec:ECGC-PG}

%\Sindri{Move the relevant text here.  More discussion of the results are needed.}


For \deleted{general} optimization with partial gradient communication\added{,} the natural generalization of error-compensated gradient algorithms \replaced{consist of the following steps:}{is to follow the steps} at 
each iteration in parallel\added{,}  worker nodes compute their local stochastic gradients $g_i(x;\xi_i)$ and \replaced{add a local error compensation term $e_i$ before applying the $\epsilon$-compressor}{compress them which accounts for the memory $e_i$}. \replaced{The}{Then, the} master node waits for all compressed gradients and \replaced{updates}{maintains} the decision vector by \deleted{performing the gradient descent step:}
\begin{equation}\label{eqn:DECCSGD}
\begin{split}
x^{k+1} &= x^k - \gamma\frac{1}{n}\sum_{i=1}^n Q(g_i(x^k;\xi_i^k) + A_i^k e_i^k), 
\end{split}
\end{equation} 
while each worker $i$ \replaced{updates its}{maintains the} memory $e_i$ according to
\begin{align*}
e_{i}^{k+1} & = g_i(x^k;\xi_i^k) + A_i^k e_i^k - Q(g_i(x^k;\xi_i^k) + A_i^k e_i^k),
\end{align*}
\replaced{Note that}{for $i=1,2,\ldots,n$. Here,} each $A_i^k\in\mathbb{R}^{d\times d}$ \replaced{only need to be available to worker $i$}{is the weighting matrix accessible only for worker $i$}. 
%
This algorithm has similar convergence properties as the error compensation for the quadradic problems \replaced{studied above.}{in the previous section (Theorem  \ref{thm:ErrorCompensatedSC}).}

\Sindri{Include definition of stochastic Hessian: call $H(x,\xi)$ stochastic Hessian if $E H(x,\xi)=\nabla^2 f(x)$ and $||H(x,\xi)-\nabla^2 f(x)||^2\leq  \mu^2 $ or $\sigma_H^2$....}



%Note that D-EC-CSGD with $A_i^k=I$ is similar to \cite{wu2018error}, and EC-CSGD is the special case of D-EC-CSGD with $n=1$. Next, we provide D-EC-CSGD convergence as shown below: 
%
%
\begin{theorem}\label{thm:distEC-CSGD_convex}
Consider an optimization problem \eqref{eqn:Problem} and the iterates $\{x_k\}_{k\in\mathbb{N}}$ generated by \eqref{eqn:DECCSGD} \replaced{under the assumption that the stochastic gradients $g_i(x^k; \xi_i^k)$ are unbiased and satisfy}{which satisfies the unbiased property~\eqref{eqn:unbiasednessSGD}  and} the bounded variance assumption~\eqref{eqn:boundedvarianceSGD}. Assume that $Q(\cdot)$ is $\epsilon-$compressor, that  $A^k_i = I -\gamma H^k_i$ where $H^k_i$ is the associated Hessian with $g_i(x^k;\xi_i^k)$, and that $e^0=0$. 
\begin{itemize}
\item [a)] If  $f$ is $\mu-$strongly convex and $L-$smooth, and \deleted{moreover} $\gamma<  (1-\beta)/(3L) $ \replaced{with}{where} $0<\beta<1$, then 
\begin{align*}
\mathbf{E}\left(f(\bar x^k) - f(x^\star) \right)
 & \leq \frac{1}{k+1}\frac{1}{2\gamma}\frac{1}{1-\beta-3L\gamma}\| x^0  - x^\star \|^2 \\ 
 &\hspace{0.4cm} + \frac{3}{2}\frac{1}{1-\beta-3L\gamma}\gamma \sigma^2,\\
  & \hspace{0.4cm} + \frac{1}{2}\frac{\mu+\frac{L}{\beta} + \left(\frac{2}{\mu}+3\gamma\right)L^2}{1-\beta-3L\gamma}\gamma^2\epsilon^2 
\end{align*}
\iffalse
\begin{align*}
\mathbf{E}\left(f(\bar x^k) - f(x^\star) \right)
 & \leq \frac{1}{k+1}\frac{1}{2\gamma}\frac{1}{1-\beta-4L\gamma}\|  x^{0} - x^\star \|^2  \\
&\hspace{0.4cm} + \frac{\mu + L/\beta + (2/\mu+4\gamma)\Lambda^2 }{2(1-\beta-4L\gamma)}\gamma^2 \epsilon^2 \\
&\hspace{0.4cm}+ \frac{2}{1-\beta-4L\gamma}\gamma\sigma^2 ,
\end{align*}
\fi
where $\bar x^k = \sum_{l=0}^k x^l/(k+1).$
\item [b)] If $f$ is $L-$smooth and $\gamma< 1/(3L)$, then 
\begin{align*}
\mathop{\min}\limits_{l\in[0,k]} \mathbf{E} \| \nabla f(x^l) \|^2 
& \leq \frac{1}{k+1}\frac{2}{\gamma}\frac{1}{1-3L\gamma}(f(x^0)-f(x^\star)) \\ 
&\hspace{0.4cm}+ \frac{3L}{1-3L\gamma}\gamma\sigma^2  + \frac{2+3L\gamma}{1-3L\gamma}L^2\gamma^2\epsilon^2  .
\end{align*}
\iffalse
\begin{align*}
\mathop{\min}\limits_{l\in[0,k]} \mathbf{E} \| \nabla f(x^l) \|^2 
& \leq \frac{1}{k+1}\frac{2}{\gamma}\frac{1}{1-4L\gamma}\left( f( x^{0}) - f(x^\star) \right) \\ 
& \hspace{0.4cm} + \frac{ {L^2} +  {\Lambda^2} + 4L\Lambda^2 \gamma}{1-4L\gamma}\gamma^2\epsilon^2 \\
&\hspace{0.4cm}+ \frac{4L}{1-4L\gamma} \gamma\sigma^2.
\end{align*}
\fi

\end{itemize}



\end{theorem}
\begin{proof}
See Appendix \ref{app:ECCGD}.
\end{proof}
\iffalse
Consider the case when $k\rightarrow\infty$ and $\nabla g_i(x;\xi_i)=\nabla f_i(x)$ (i.e. $\sigma^2=0$ and $N=0$).  D-EC-CSGD reduces quantization error by $\mathcal{O}(\gamma^2)$, unlike D-CSGD. In addition, 
\fi
%
%
%
%
%
% 
This theorem shows that error compensation in D-EC-CSGD can \replaced{attain}{recover} arbitrarily high solution accuracy  unlike \added{the} direct compression \replaced{analyzed}{as shown} in Theorem \ref{thm:distCSGD_convex}. In particular, error compensation has \replaced{a residual}{quantization} error which is bounded by $\mathcal{O}(\gamma^2)\epsilon^2$. Therefore, the residual error related to both stochastic gradient noise $\sigma$ and precision of quantization $\epsilon$ can \replaced{by made arbitrarily small by decreasing the step-size.}{diminish toward zero with diminishing step-size from Theorem \ref{thm:distEC-CSGD_convex}. }

{\color{blue}
	I have come this far. I believe that the paragraph below needs to be expanded and our contributions must be emphasized even more clearly (unless they are repeated in subsection C below.)
	
	Please go over the document for consistency of notation. We now have $\epsilon$-compressors, $\epsilon$-DBEC compression, and $\epsilon$-deterministic compressions. Please use only one of these terms! Also, there is a footnote we should remove so that we do not forget it.	
}
When we let  $\Lambda = 0$  in Theorem \ref{thm:distEC-CSGD_convex}, we \deleted{can also} recover the convergence results of D-EC-CSGD using error compensation variants with $A_i^k=I$ proposed by \cite{alistarh2018convergence,wu2018error}\replaced{. However, in contrast to earlier results, our proof requires neither}{ without} the mergeability assumption \replaced{or}{nor} unbiasedness of \deleted{the} compression operators (\replaced{cf.}{see \emph{e.g.}, in} \cite[Assumption 1]{alistarh2018convergence} and \cite[Lemma 1]{wu2018error}, respectively).
 %Furthermore, we establish convergence results of D-EC-CSGD using error compensation proposed by~\cite{ourICASSPworks} when we let $H_i^k$ be Hessian information associated with the stochastic gradient $\nabla g_i(x^k;\xi_i^k)$.
%{\color{blue} I do not understand the last sentence in the above paragraph.}


\subsection{Comparison with Other Error Compensation Schemes} \label{subsec:Comparisons}
%
%\Sindri{In the introduction we mentioned that   \cite{alistarh2018convergence,ourICASSPworks,wu2018error,Stich2018,2019arXiv190109847P,tang2019doublesqueeze,tang2019texttt} are all error-compensation mehtods. Why are thy not all mentioned here? Also we discussed methods that had scaled $A$ equal to scaled identity matrix. No need to do the math for all of these, but they should be mentioned.}
%
We now compare our algorithm and results with the other recent works on error compensation, \cite{alistarh2018convergence,wu2018error,Stich2018,2019arXiv190109847P,tang2019doublesqueeze,tang2019texttt}. 
%
The error compensation in all of the previous papers keeps in memory the sum (or weighted sum) of all previous compression errors. 
 We can \replaced{write all}{express} these error \replaced{compensation schemes}{compensations} in the form of \deleted{our algorithm in} Equation~\eqref{eqn:DECCSGD} (Section~\ref{subsec:ECGC-PG}) by setting $A_i^k =  I$ (or $A_i^k =  \alpha I$ for some $\alpha\in(0,1)$). If we perform the same convergence analysis on this error compensation as we did for the centralized algorithm  for \deleted{the} quadratic problems in Section~\ref{subsec:ECGC-AII}, then we have 
\begin{align*}
x^{k+1} - x^\star & = A_\gamma^{k+1}(x^0-x^\star) + \gamma e^{k+1} - \gamma^2 \sum_{l=0}^{k} A_{\gamma}^{k-l} H e^l,
\end{align*}
where $A_\gamma = I - \gamma H$. 
 The final term shows that these error compensation schemes do not remove the accumulated compression errors, even though they have been shown to outperform direct compression.
%Even though this existing error compensation scheme has been shown to outperform direct compression, it \replaced{does not}{cannot entirely} remove the accumulated quantization errors.
However, our error compensation does remove all of the accumulated error, as shown in Section~\ref{subsec:ECGC-AII}. This \replaced{example}{intuition} shows why Hessian-based error compensation can be more \replaced{effective}{competitive} than the existing scheme\replaced{s.}{ since it avoids accumulations of all quantization errors as shown in subsection~\ref{subsec:ECGC-AII}. }
%
%
%
%
%Unlike direct compression, Hessian-based error compensation helps remove accumulation of quantization errors. Simultaneous to our work, Karimireddy \emph{et. al} \cite{2019arXiv190109847P} present the convergence analysis of stochastic gradient descent using the existing error compensation variants studied, \emph{e.g.} in \cite{alistarh2018convergence,wu2018error,Stich2018}. However, the analysis is restricted to the centralized architecture.  Tang \emph{et. al} \cite{tang2019doublesqueeze} propose double-pass compression using this existing error compensation which save the significant number of communicated bits. Their results apply for randomized compression operators without unbiased property requirements.

%However, our theorems readily establish unified results of this error compensation variant for both centralized and distributed architectures when we let $A_i^k=I$ in the update in Equation~\eqref{eqn:DECCSGD} (or equivalently let $\Lambda = 0$  in Theorem \ref{thm:distEC-CSGD_convex}). 
We validate the superior performance of Hessian-based error compensation over \deleted{the} existing \replaced{schemes}{counterpart} in Section~\ref{sec:numericalresults}. To \replaced{reduce computing and memory requirements}{save Hessian computations}, we \deleted{also} propose \replaced{a Hessian}{the diagonal} approximation (\deleted{i.e. }\replaced{using}{keeping} only the diagonal elements of the Hessian)\deleted{ which leads to \replaced{a}{the} computation cost of $\mathcal{O}(d)$}. \replaced{Error compensation with this approximation}{This diagonal Hessian error compensation} is shown to have comparable performance to \replaced{using the full Hessian.}{its full Hessian-based counterpart. }





%However, we show that the error compensation scheme motivated by \cite{ourICASSPworks} ($H_i^k$ is the Hessian information associated with the stochastic gradient $\nabla g_i(x^k;\xi^k_i)$) outperforms others when the binary compression is used in the next section.






